Efficient NLP Model Finetuning via Multistage Data Filtering

As model finetuning is central to the modern NLP, we set to maximize its efficiency. Motivated by redundancy in training examples and the sheer sizes of pretrained models, we exploit a key opportunity: training only on important data. To this end, we set to filter training examples in a streaming fashion, in tandem with training the target model. Our key techniques are two: (1) automatically determine a training loss threshold for skipping backward training passes; (2) run a meta predictor for further skipping forward training passes. We integrate the above techniques in a holistic, three-stage training process. On a diverse set of benchmarks, our method reduces the required training examples by up to 5.3$\times$ and training time by up to 6.8$\times$, while only seeing minor accuracy degradation. Our method is effective even when training one epoch, where each training example is encountered only once. It is simple to implement and is compatible with the existing finetuning techniques. Code is available at: https://github.com/xo28/efficient- NLP-multistage-training

==> CamRd_IJCAI_efficient_NLP_Latex/abs.tex <==
% !TeX root = main.tex
% --- Xu's version -- 

\begin{abstract}

% Most of the prior work has focused on designing compact models or reducing weights computations to increase the finetuning efficiency.
% \annote[YJ]{efficient model structures or searching for an efficient substitution}{I am not sure what do you mean by "efficient model structures" or "efficient substitution"}
% Complementary to them, we exploit a largely ignored opportunity which is the efficient use of training data. 
% Previous works show that the training examples are often redundant, duplicated, and noisy.
% In this paper, we examine the problem of searching for the most important data instances by model losses to maximally benefit learning. Specifically, we update a loss threshold and a predictor with model loss to filter out unimportant data.
% To overcome the unnecessary of observing the entire training process, 
% we propose the Automatic Threshold method and the Three-stage Training mechanism, which would update a lightweight classifier along with the main model being trained in the Online Learning fashion.
% % \xzlNote{update the following with result highlights.}
% On a diverse set of benchmarks, our algorithm reduces the total training time by up to 6.7$\times$ with 0.74\% accuracy degradation on average. Ours also skips forward passes for up to 81\% training examples when training for 2 epochs. As the epoch count grows, our efficiency is increasingly higher, e.g. up to 18.1$\times$ training time reduction at 1.83\% accuracy degradation when training for 5 epochs. 

% With neglectable computing overhead, the proposed methods deliver comparable performance with DistillBERT model on four NLP datasets of different tasks. Experiments show our methods achieve great accuracy-efficiency trade-off.
% \note[YJ]{Despite of some writing issues, this abstract basically contains what it needs to have. To reduce the length, maybe we can leave out some technical details --- which we can discuss later.}

% \xzlNote{please compare to the revision below}

As model finetuning is central to the modern NLP, we set to maximize its efficiency. 
Motivated by redundancy in training examples and the sheer sizes of pretrained models, we exploit a key opportunity: training only on important data. 
To this end, we set to filter training examples in a streaming fashion, 
in tandem with training the target model. 
Our key techniques are two: (1) automatically determine a training loss threshold for skipping backward training passes; 
(2) run a meta predictor for further skipping forward training passes. 
We integrate the above techniques in a holistic, three-stage training process. 
% Incarnated as a three-stage process, 
On a diverse set of benchmarks, our method reduces the required training examples by up to 5.3$\times$ and training time by up to 6.8$\times$, while only seeing minor accuracy degradation. 
% \xzlNote{why not talking about training time reduction as well?}
% \annote[YJ]{0.74\% accuracy}{can we use ``minor'', my concern is that readers may misunderstand this} . 
Our method is effective even when training one epoch, where each training example is encountered only once. 
It is simple to implement and is compatible with the existing finetuning techniques. 
Code is available at: \href{https://github.com/xo28/efficient-NLP-multistage-training}{https://github.com/xo28/efficient-NLP-multistage-training}
% \annote[YJ]{finetuning optimizations}{not sure layer freezing can be called finetuning optimization} such as layer freezing. 
\end{abstract}

\xzlNote{}

==> CamRd_IJCAI_efficient_NLP_Latex/ack.tex <==
\section*{Acknowledgments}
The authors were supported in part by NSF awards \#2128725, \#1919197, \#2106893, \#2124538, and Virginia's Commonwealth Cyber Initiative.
The authors thank the anonymous reviewers for their insightful feedback.

==> CamRd_IJCAI_efficient_NLP_Latex/discussion.tex <==
\section{Discussion on Design Choices}

\label{sec:discussion}


\subsection{Automatic loss thresholds}
\vspace{-1mm}
%\textbf{Theoretical justification...} \xzlNote{Yangfeng: add as you see fit}

\paragraph{Loss for filtering data}
We use losses for the following reasons. 
(1) 
As shown in prior work~\cite{loshchilov2015online}, 
losses effectively reflect model update from given examples: 
higher loss means that the model makes higher inference errors and hence can learn more from this example. 
%(2) 
%Prior work on selecting training data uses loss ... among other metrics (e.g. gradients, similarity of training set vs. dev set) 
(2) 
%Losses well suit our efficiency goal: they incur 
Getting losses is computationally inexpensive: they incur no computation overhead beyond forward passes. 

\paragraph{Rationales for a loss threshold} 
We want to selectively learn from a subset of examples with the highest losses. 
To identify such a subset, one may attempt to compare the losses of all training examples.
This however suffers from two drawbacks.
(1) It is inefficient: doing so requires forward passes on \textit{all} the training data, an expensive task with poor data locality, 
because the activations calculated by forward passes must be saved to disk and later restored for executing backward passes. 
(2) As a model is being updated, the losses of examples yet to be trained will  change. 
For instance, a previously high-loss example (estimated by the untrained model) may see a low loss and hence is no longer worth training. 



%Specifically, for a given input data point, if its loss is larger than the threshold $L_{low}$, we consider the model doesn't perform well on this data, so we will keep it and update the model by doing back-propagation as usual. On the other hand, if the loss of the input data is lower than $L_{low}$, we consider the model has been already well trained in the pre-training and we can skip this data.

By contrast, we use a loss threshold to screen examples. 
(1) The method is effective because it accommodates continuous model updates. 
As the loss is always assessed based on the updated model, the method estimates how much the \textit{updated} model can learn from the example under question. 
(2) The method is efficient because it consumes training data sequentially with good locality; it is, therefore, friendly to memory hardware hierarchy. 
(3) The method leads to self-paced training. 
As training starts, the model likely sees high losses on most data, for which it will filter less; as training goes on and the model is updated, it likely sees lower losses on more data, for which it will filter more. 

\paragraph{Tradeoffs for setting a loss threshold} 
Ideally, we want to train on the fewest examples and have an accuracy close to that from the \textit{TrainAll} baseline. 

Hand-picking $L_{low}$ is tricky: 
a $L_{low}$ too high can be overly \textit{passive}~\cite{shalev2003online}, 
resulting in too much data filtered and suboptimal accuracy; 
a $L_{low}$ too low can be overlay \textit{aggressive}, resulting in long training delays. 
The optimal choice of $L_{low}$ hinges on a discrepancy between the model's knowledge prior to training and the total knowledge encoded in the training data. 
%Therefore, $L_{low}$ is specific to the pretrained model as well as the training data. 
Unfortunately, this discrepancy cannot be accurately determined until we have trained on all the data. 
This motivates us to derive $L_{low}$ automatically.

\paragraph{Automatic loss thresholds}
%We derive $L_{low}$ automatically from on a small sample of the training data. 
%The mechanism is as follows. 
%The trainer pre-shuffles all training data randomly. 
%As it runs it maintains a sliding window, which consists of losses of most recent $w$ examples. 
%The trainer sets $L_{low}$ to be the mean of the sliding window. 
We set $L_{low}$ to be the average of the most recent losses for the following reasons.
(1) By considering a sample of the total training set, the average loss estimates how the current model fits the data yet to be trained with; 
(2) By picking $L_{low}$ to be the \textit{average} loss, we balance being passive and being aggressive in filtering examples. 
(3) We keep updating $L_{low}$ in sliding windows so that we keep refreshing the estimation.
%(4) Since $L_{low}$ is estimated on already seen data, the updated model in using $L_{low}$ will be more selective. 
\vspace{-1mm}
\subsection{The loss predictor}
\vspace{-1mm}
%While loss suggests if an example is worth training, it nevertheless requires a forward pass to run on this example. 
%To eliminate the computation cost for the forward passes, can we predict the loss of an training example  \textit{without} the forward pass?

%The challenges are twofold. 
%First is what features should the predictor be based on.
%%To have significant cost reduction, 
%That extraction of such features must be significant cheaper than a forward pass of the language model $M$ under training. 
%Second is who is responsible for training such a predictor, which shall be specific to the model $M$ and the training data? 

Our meta predictor addresses two design questions. 
First, what features should the predictor be based on?
That extraction of such features must be significantly cheaper than a forward pass of the language model $M$ under training. 
We adopt Bag-of-Words (BoW) features of an input sequence as input of the predictor. Bag-of-words is one of the classical text features for different NLP models and tasks~\cite{sebastiani2002machine,heckerman1997bayesian,lewis1998naive}.
%, including the naive Bayes model
Apart from BoW features, other text classification features can also be used.
%Intuitively, a language model is more likely to err on a sentence containing rare words, hence should train with the sentence with a higher probability. 

Second, who is responsible for training the meta predictor, which shall be specific to the model $M$ and the training data? 
We train the predictor under the supervision of loss-based example filtering (stage 1). 
The training does not have to be long before the predictor can be queried to make predictions and advise on filtering training data. 


It is worth noting that even when the trainer queries the predictor for  filtering decisions (stage 2), it still updates the predictor continually.  % opportunistically. 
This is done on the data that the predictor deems worth training: 
the trainer runs forward passes on such data, get the losses, and uses the comparison outcome to update the predictor. 
This keeps the predictor updated to the changing language model $M$: 
as $M$ is being trained, the correlation between its loss on new data and the data's BoW features is drifting; 
intuitively, $M$ will see a lower loss given the same BoW features. 

The cost of meta predictor training (naive Bayes) is two orders of magnitude lower than the target model (DistillBERT). 
% On our Nividia GPU, it’s 24.13$\times$ lower on SST2. The meta predictor training takes 53s and DistillBERT training takes 1279s.
%
As stated in \S\ref{3stages}, training stops when the meta predictor’s average loss drops below a threshold, ALT. Section \S\ref{hyperparameters} further tests a range of ALT values. 



\begin{comment}  % ----- xzl: not much useful info
\subsection{Complexity analysis of our method}
{\color{blue} There are two dimensions of complexity analysis of our method: (1) the fraction of skipped training computation under the redundancy assumption. (2) the worst-case guarantee: that our method will perform as well as training with all the data, in case of no data redundancy. 
% \input{tab-complexity.tex}

As shown in Table \ref{tab:e2e-combined}(a), our method is able to achieve comparable accuracies with TrainAll. In Table \ref{tab:e2e-combined}(b), we show that these accuracies can be achieved by skipping a large portion of training data.


If there is no data redundancy, the data losses will be big because they are hard for the model’s capacity. Since the model will be updated with the previous data, the corresponding loss threshold will get lower during training. Therefore, the coming data which have higher losses will not be filtered, so they will be all included in the coreset to train the model. Our method is guaranteed to perform as well as train with all the data.}
\end{comment}

==> CamRd_IJCAI_efficient_NLP_Latex/eval.tex <==
% !TeX root = main.tex


\section{Evaluation}
\label{sec:eval}
\vspace{-1mm}
We set to answer the following questions: 
\begin{myitemize}
\item Compared to the existing training method, 
can we achieve comparable accuracy with much higher efficiency? 
\item How significant are our key techniques?
\item How sensitive is our method to its hyperparameters and what are their reasonable ranges?
\end{myitemize}

\vspace{-1mm}
\subsection{Experiment Setup}
\vspace{-1mm}
% The proposed method is evaluated on four NLP tasks, ranging from sentiment analysis to Question-Answering task, with DistillBERT models.

\paragraph{Models \& Datasets}
We test our method on the pretrained DistilBERT model with 6 transformer layers and a hidden dimension of 768. 
We finetune it on five classification benchmarks.
% \xzlNote{only cite GLUE, not the individual benchmarks (except AMZ)}
Three are from GLUE \cite{wang2019glue},
% (SST2 \cite{socher2013recursive}, QNLI \cite{rajpurkar2016squad}, QQP \footnote{https://data.quora.com/First-Quora-Dataset-Release-Question-Pairs})
one is the Amazon Polarity (AMZ) \cite{zhang2015character}, and one multilabel benchmark is AG News (AG) \cite{Zhang2015CharacterlevelCN}
The benchmarks cover tasks of single-sentence, similarity, and inference. 
All the benchmarks have substantial training data, allowing opportunities for filtering. 
For the three GLUE benchmarks, we reproduce the accuracies reported in prior work \cite{sanh2019distilbert} and consider them as the baseline performance; 
for Amazon Polarity and AG\_news, we finetune the model and report accuracy measured on its test set.
We choose these datasets by following DistillBERT's experiment plan and they are substantially large. Our methods only rely on losses and semantic information. Therefore, they can be easily applied to various NLP tasks by loading different pretrain models.
The comparable efficacy of batch and example skipping prompted our inclusion of results from the latter approach.

% We test our method on the pretrained DistilBERT model with 6 transformer layers and a hidden dimension of 768. 
% We finetune it on four classification benchmarks as summarized in \autoref{tab:data-statistics}. 
% % \xzlNote{only cite GLUE, not the individual benchmarks (except AMZ)}
% Of these benchmarks, three are from GLUE \cite{wang2019glue}
% % (SST2 \cite{socher2013recursive}, QNLI \cite{rajpurkar2016squad}, QQP \footnote{https://data.quora.com/First-Quora-Dataset-Release-Question-Pairs})
% and one is the Amazon Polarity (AMZ) \cite{zhang2015character}.
% The benchmarks cover tasks of single-sentence, similarity, and inference. 
% All the benchmarks have substantial training data, allowing opportunities for filtering. 
% For the three GLUE benchmarks, we reproduce the accuracies reported in prior work \cite{sanh2019distilbert} and consider them as the baseline performance; 
% for Amazon Polarity, we finetune the model and report accuracy measured on its test set.
% We choose these datasets by following DistillBERT's experiment plan and they are substantially large. Our methods only rely on losses and semantic information. Therefore, they can be easily applied to various NLP tasks by loading different pretrain models.

\iffalse
\begin{table}
\centering
\begin{tabular}{llllll}
\hline
\textbf{Datasets} & \textbf{Tasks} & \textbf{\#train} & \textbf{\#dev} & \textbf{\#test} \\
\hline
SST2 &sentiment& 67k & 0.9k & 1.8k \\
QNLI & QA/NLI & 105k & 5.5k & 5.4k \\
QQP & paraphrase& 364k & 40k & 391k \\
AMZ & sentiment& 3600k & N/A & 400k \\
AG & topics & 120k & N/A & 7.6K \\
\hline
\end{tabular}
\caption{\label{tab:data-statistics} Statistics for datasets, which are all binary classification tasks and \# counts the number of examples in the train/dev/test sets.}
\end{table}
\fi

\paragraph{Baselines} 
% As the goal of our work is to propose a novel training data skipping mechanism that boosts the efficiency and maintain a comparable accuracy, 
We evaluate against four groups of baselines. 
(1) \textit{TrainAll} trains models with all the training data.
(2) \textit{FixedThreshold} filters the training data with hand-picked, fixed loss thresholds, for which we sweep the range $[0.1,0.7]$ at an increment of 0.2. 
% the hope is to identify a close-to-optimal threshold for each benchmark.
(3) \textit{AutoAssist}~\cite{zhang2019autoassist} filters out instances with a lightweight ``assistant'' model jointly with the target ``Boss'' model. The assistant selects and generates batches during training both models. 
(4) \textit{Selection via Proxy} (SVP)~\cite{coleman2019selection} uses a small proxy model to perform core-set selection and train the target model with the core-set.

% \xzlNote{the following weak}}

% We evaluate our method against two groups of baselines. 
% (1) \textit{TrainAll} trains models with all the training data.
% (2) \textit{FixedThreshold} filters the training data with hand-picked, 
% fixed loss thresholds, for which we sweep the range $[0.1,0.7]$ at an increment of 0.2; the hope is to identify a close-to-optimal threshold for each benchmark.
% \xzlNote{the following weak}
% We don't compare with other methods because they are for model pretraining not finetuning. This is same for methods similar to ours, like AutoAssist \cite{zhang2019autoassist}. It needs to train many more epochs than us to work normally..

% \xzlNote{Figure 3: the blue/red circles will be indistinguishable on monochrome printout. Change one of them}

\input{tab-hyperparam}

\paragraph{Metrics}
For a training process, we report (1) the model accuracy after training and (2) the training time, which is inverse to training efficiency. We make experiment results reproducible. 
% \xzlNote{below: state what is measured on our machine; what is estimated/calculated and can be extrapolated for a diff machine...}
On our machine with Nvidia RTX 2080 Ti, % and Intel 10 core CPU, 
we measure the time of a forward pass ($T_f$) and a backward pass ($T_b$), as well as the fractions of data on which only backward passes are skipped ($\alpha_b$) and \textit{both} forward and backward passes are skipped ($\alpha_{fb}$) in each training process. 
For a given training process, the total time is $T=\alpha_b T_f + (1-\alpha_b-\alpha_{fb}) (T_f + T_b)$. 
Finally, we normalize $T$ to that of \textit{TrainAll} as
$T_{norm}= \frac{T_{ours}}{T_{all}}$ and report $T_{norm}$.


\input{fig-pareto}


\input{tab-e2e-combined}

\vspace{-1mm}
\subsection{End-to-end results}
% \vspace{-1mm}
\autoref{fig:pareto} plots accuracy versus training time. 
It shows that our method delivers both high accuracy and high efficiency (i.e. low training time). 
Compared to \textit{TrainAll}, our method reduces the training time by at least 2$\times$. 
Meanwhile, the accuracy is similar: 
on QNLI, our best accuracy is only about 1\% lower than that of \textit{TrainAll};
on QQP, AMZ, and AG, our accuracy is within 1\% of that of \textit{TrainAll}. 

Note that on SST2 our accuracy is even higher than \textit{TrainAll}, 
which we attribute to that our method excludes training examples that the model is already confident about, therefore preventing overfitting on such examples. 

% Our algorithm sometimes achieves better accuracy than standard fine-tuning because ours excludes the data points the model is confident about. It'll be hard for the model to handle hard cases if it has overfitted on those easy samples.


% \xzlNote{XXX, or on average??} XXX percentage point across all the benchmarks. 
%Notably, the best accuracies delivered by our method are within 0.02\%/0.2\% on SST2/AMT respectively; 
%the accuracies are superior on benchmark QQP and QNLI, likely because noisy training data is filtered. 
% As the performances shown on SST2 and AMZ, the best accuracy among them could achieve almost the same accuracy (with gap of 0.02\% and 0.2\%, respectively) as TrainAll. 

% Pareto-optimal 
Our method provides rich trade-offs between training accuracy and efficiency. 
\autoref{fig:pareto} highlights a series of \textit{Pareto} results as desirable trade-offs~\cite{deb1999multi}: 
given a result, no other result has both higher accuracy and higher efficiency. 
% \autoref{fig:pareto} plots accuracy versus training time. 
% It shows that our method delivers both high accuracy and high efficiency (i.e. low training time). 
% Compared to \textit{TrainAll}, our method reduces the training time by at least 2$\times$. 
% Meanwhile, the accuracy is similar: 
% for SST2, QQP, AMZ, all our performances are within 1\% of \textit{TrainAll}'s accuracies, some are even higher than \textit{TrainAll}.
% QNLI's best accuracy is only about 1\% lower than that of \textit{TrainAll}, which is comparable.
% % \xzlNote{XXX, or on average??} XXX percentage point across all the benchmarks. 
% %Notably, the best accuracies delivered by our method are within 0.02\%/0.2\% on SST2/AMT respectively; 
% %the accuracies are superior on benchmark QQP and QNLI, likely because noisy training data is filtered. 
% % As the performances shown on SST2 and AMZ, the best accuracy among them could achieve almost the same accuracy (with gap of 0.02\% and 0.2\%, respectively) as TrainAll. 

% % Pareto-optimal 
% Our method provides rich tradeoffs between training accuracy and efficiency. 
% \autoref{fig:pareto} highlights a series of \textit{Pareto} results as desirable tradeoffs~\cite{deb1999multi}: 
% given a result, no other result has both higher accuracy and higher efficiency. 

\paragraph{Accuracy gain over time (AGOT).}
% In some situations, 
Prior efficient training research often compares accuracies under a fixed computation budget and vice versa. 
Yet, using a single evaluation metric can be inadequate, as neither accuracy or runtime could characterize the tradeoffs between them in a comprehensive fashion.
To this end, a user may want to quantify her most desirable accuracy/efficiency tradeoff. % and compare it to alternative methods. 
We therefore define AGOT: 
% a metric that captures both the model accuracy and the training time. 
\vspace{-1mm}
\begin{equation}
\label{eq:agot}
\text{AGOT}_{\varepsilon}(a, t) = \frac{a - a_{base}}{a_{full} - a_{base}}\cdot \frac{1}{T_{norm}^{1-\varepsilon}}
\end{equation}
where $a$ is the model accuracy after training and $T_{norm}$ is the training time normalized to \textit{TrainAll}; 
$a_{base}$ and $a_{full}$ are model accuracies before training and after training with all the data, respectively. 
In the above definition, the accuracy gain (the first term) is inversely weighted by the running time needed to achieve this gain (the second term). 
The parameter $\varepsilon\in[0,1]$ is decided by the user, 
reflecting her preferred importance of accuracy with regard to the training time. 
% balancing the importance of accuracy and that of the time. 
A larger $\varepsilon$ weighs more on the accuracy; 
a special case $\varepsilon=1$ means not considering the time at all.
Specifically, we set $\varepsilon=0.95$, weighting significantly on the accuracy: 
a few points of accuracy gain often warrants significantly longer training time as shown in \autoref{fig:pareto}. 

To compare against baselines, for each benchmark we consider the result with the highest AGOT score, referred to as AGOT-optimal. 
As shown in \autoref{fig:pareto}, AGOT effectively identifies accuracy/efficiency sweet spots. 
On QNLI and QQP, the AGOT-optimal results are the ones with the highest accuracy among all the results with slightly longer training time than the latter.
On AMZ and AG, the AGOT-optimal result has slightly lower accuracy 
%than the best (94.08--94.81, 1.16\% lower than \textit{TrainAll}) 
but much lower training time. % than the later (46\% on average).
The AGOT-optimal results are highly competitive against \textit{TrainAll}. 
Take SST2 as an example, the AGOT-optimal reduces the training time by 85\% while showing superior accuracy by 0.69\%, likely because noisy training data is filtered. 
% Notably, the best accuracies delivered by our method are within 0.02\%/0.2\% on SST2/AMT respectively; 
% the accuracies are superior on benchmark QQP and QNLI, likely because noisy training data is filtered. 
%On QNLI and QQP, the AGOT-optimal result is the one with the highest accuracy (1.04/1.44) among all trade-offs with slightly longer training time than them (still 67\% and 62\% shorter than \textit{TrainAll}). 
%On AMZ, the AGOT-optimal result has slightly lower accuracy than the best trade-off (94.08--94.81, 1.16\% lower than \textit{TrainAll}) but significantly lower training time than the later (46\% on average). 

We next focus on AGOT-optimal results. 

%On SST2, its accuracy is only lower by 0.13\% \xzlNote{higher???} while its 
%This also prove the effectiveness of our method that the model benefits from training with the important data, which actually let the model only focus on more essential features.

%One interesting observation is the AGOT selected hyperparameter setting in AMZ --- when other prediction accuracy is sufficiently high, the AGOT score prefers to select the setting with the least running time (the lowest value along x-axis).
%While in an opposite case (QNLI), it prefers to select the setting with the highest accuracy, even it may cause a little compromise on the computational efficiency.
%
%Dots on the Pareto front are considered equally good, so our method can give many desirable candidates. 

\paragraph{How much computation is skipped?}
Our method skips large fractions of forward and backward passes. 
As \autoref{tab:e2e-combined} (b) shows, across all benchmarks, on 52.87\% -- 81.01\% of the training data both forward and backward passes are skipped. 
% Such fractions are significantly higher than that of training data on which backward passes are skipped while forward passes are executed (8.95\% on average).
%the fraction of skipped backward only passes is lower  (from stage 1 and stage 2) yet noticeable, 8.95\% on average.
This indicates that our predictor, which controls skipping both forward and backward passes, is highly effective. 
In addition, on 8.95\% of the training data on average, backward passes are skipped while forward passes are executed. 

\paragraph{Comparison versus prior works}
% We compare with AutoAssist \cite{zhang2019autoassist} and Selection via Proxy (SVP) \cite{coleman2019selection} because they are methods similar to ours. 
% \xzlNote{Proof read below}
The results are shown in Table~\ref{tab:e2e-combined}.
Compared to \textit{AutoAssist}, our method trains for much less time (up to 5.33$\times$) while achieving similar/higher (-0.13\% -- +0.46\%) accuracy.
AutoAssist's disadvantage is likely because its choices of filtered data is sub-optimal:
a large fraction of training batches are generated via random selection with replacement,
which forces the simple assistant model to learn duplicate samples. 
Furthermore, since the assistant is being updated throughout the whole training process,
overfitting is likely to occur.

% --- Xu's ----
%Both our accuracy and efficiency outweigh those of AutoAssist consistently across three GLUE benchmarks and the Amazon Polarity dataset. 
%We achieve 0.22\% -- 0.46\% accuracy increment and reduce as high as 5.33$\times$ training time. On AG news, we have comparable accuracy which is 0.13\% lower AutoAssist and even only 0.05\% gap between \textit{TrainAll}. But we can finish training 2.6$\times$ faster with such close performance. We speculate the superior comes from that AutoAssist can reduce the redundancy inside the whole dataset while having redundancy inside the filtered data. A large part of the batches is generated by random selection with replacement, which actually hurts the trained Assistant model during late training. Besides, the very simple Assistant model will be updated throughout the whole training process making it overfitting easily.

We evaluate \textit{SVP} on AMZ and AG (not in Table~\ref{tab:e2e-combined}),
as SVP's data preparation code is incompatible with the remaining benchmarks. 
On the benchmarks, SVP's accuracies are 88.54 and 90.02, respectively; 
the normalized training times are both 0.4.
Compared to SVP, our method's accuracies are 5.54\% and 3.62\% higher and our training time is  1.82$\times$ and 2.67$\times$ shorter. 
This is because SVP's core-set selection depends on the consensus of data valuation between the proxy and the target models, which does not always hold. 
% The data selection intertwined with model training in our method leads to more straightforward benefits.


% ----- Xu's ----------
%Due to the data preparation process of SVP, we don't compare its performances on GLUE benchmarks. We reproduce its performances on Amazon Polarity and AG News datasets and have the accuracy/normalized run time numbers: 88.54/0.4 and 90.02/0.4. Our three-stage method achieves 5.54\% and 3.62\% accuracy improvement and accelerates training by 1.82$\times$ and 2.67$\times$. The large accuracy gap resulting from the core-set selection in SVP highly depends on the consensus of data valuation between the proxy and the target model. However, it is not guaranteed. The data selection intertwined with model training in our method leads to more straightforward benefits.

%By comparison, the filtering is more conservative in earlier stages before the predictor is trained.  
%the fraction of skipped backward only passes is lower  (from stage 1 and stage 2) yet noticeable, 8.95\% on average.
%It also proves our method skips less at the beginning of training and be more aggressive after a classifier is trained.

% \xzlNote{instead, say that as more epochs are trained, our efficiency (efficiacy of filtering) will be more pronounced, as will be shown in Section XXXX}
% A breakdown of three stages: their splits, fraction of examples skipped, fraction of compute reduced. 

%\paragraph{Memory saving}
%We reduce accumulated memory consumption over time but does not reduce peak memory consumption, which is determined by the M (the number of layers, the memory footprint of activations per layer) that we do not change. 

It is worth noting that 
both \textit{AutoAssist} and \textit{SVP} need to train significantly more epochs than ours. 
For example, AutoAssist needs 100 epochs on image and language tasks. 
%Furthermore, our overhead is lower. While our meta predictor only needs to learn in stage 1, the assistant and proxy models must do so throughout the whole dataset.

\iffalse
We train the same number of epochs and measure the post-training accuracy A as well as the runtime T. 
Lower runtime means higher efficiency. 
We normalize all runtimes to the runtime of training with Vanilla. 
We test different combinations of hyperparameters as listed in Table XXX. 
Each combination will yield a pair <A, T> with variation. 
To pick the most favorable (representative?) results, we define a unified metric summarizing <A,T> pair. 
The metric is accuracy gain over time (AGOT): 
AGOT = ... 
Specifically, the accuracy gain is normalized to the gain of the Vanilla baseline, indicating the fraction of achievable accuracy gain, i.e. training progress. 
From results in Figure XXX, we select the ones with the highest AGOT and and present them in Table XXX. 
The results show that over four benchmarks, our method reduces the total training time by XXX while only see XXX lower accuracy. 
We illustrate all such pairs in Figure XXX--XXX. 
In these figures, any point on the Pareto front is valid (? Pareto optimal) -- no other point has both more accurate and more efficient (i.e. has lower runtime). 
Each plot contains multiple such points; they all take significant shorter runtimes (XX\%--XX\%) and only see accuracy lower by XXX\%. 
\fi



\paragraph{Estimated energy \& CO$_2$ reduction}
% \xzlNote{power vs energy}
%We further estimate the reduction in training energy and CO2 emission. 
We use an energy model~\cite{strubell2019energy}: 
\vspace{-1mm}
\begin{equation}
\begin{split}
&p_t = \frac{1.58t(p_c+p_r+gp_g)}{1000}; CO_2e = 0.954p_t
\end{split}
\end{equation}

In the equation, $p_t$ is the total energy consumed during finetuning, $p_c$ is the average CPU power draw, $p_r$ is the average DRAM power draw, $p_g$ is the average GPU power draw, $t$ is the training time, and $g$ is the GPU count. 
% \xzlNote{the model does not show energy?}
% Finetuning in SST2 then plug in our training time and power draws.
%We consider energy consumption of compute (e.g. GPU) and memory access. 
Compared to \textit{TrailAll}, we reduce the total energy consumption by 45.85\% on average across all benchmarks. 
%This conversion takes into account the relative proportions of different energy sources (primarily natural gas, coal, nuclear and renewable) consumed
%to produce energy in the United States. Based on this,
% Assuming such power is generated through coal,
Considering the proportions of different energy sources in the US~\cite{strubell2019energy}, 
we estimate to reduce the CO$_2$ emission from 1.05 pounds per training process to 0.56 pounds on average.


%\input{tab-accuracy}
% \input{fixed}
% \input{tab-baselines}
%\input{tab-e2e}
%\input{tab-skipratio}

\input{tab-epochs}

% \input{fig-pareto}

%\input{sst2-pareto}
%\input{qnli-pareto}
%\input{qqp-pareto}
%\input{amazon-pareto}

\input{tab-random}


% \xzlNote{Table 4: make it consistent with Table 3}
\vspace{-1mm}
\subsection{Ablation Study}
\vspace{-1mm}
%\subsection{Significance of key designs}
%We next present breakdown and ablation studies. 

%\paragraph{Quantitative results.}
%\autoref{tab:platform}, \autoref{tab:skipratio}, and \autoref{fig:epochs} report the quantitative results associated with the settings selected by the AGOT score.



\paragraph{Efficacy of using loss thresholds}
%Table~\ref{tab:cmp-random} shows that loss thresholds can effectively filter data that has low impact on training accuracy. 
The results are shown in Table~\ref{tab:cmp-random}. 
Compared to filtering the same amount of training data that is randomly selected,
% \xzlNote{how are these defined? fwd? bwd?} 
%(i.e. the same training time), 
methods based on loss thresholds show consistently higher accuracies. 
Specifically, \textit{FixThreshold} with loss thresholds of $[0.1, 0.3, 0.5]$ (the skip ratio varies from 20.72\% to 83.25\%) shows accuracies higher by 0.93\% -- 1.33\% on average.
% \{0.93\%,1.55\%,1.33\%\} on average.
The Three-stage method shows accuracies higher by 
% 0.89\%--4.13\% and
2.14\% on average.
Note that such accuracy improvement is significant:
% \xzlNote{the following sentence: why use .23? our accuracy is higher by 2\%, we should use a number near 2\%.}
take Figure~\ref{fig:pareto} as reference, one can reduce the training time by 5$\times$ with tolerating accuracy drop as low as 2.01\% by average.
% \xzlNote{Table 6: put the dox in. Beautify it.}

%It shows that FixThreshold achieves higher accuracies across all the datasets when the threshold equals to 0.1, 0.3, and 0.5. These thresholds cover a wide range of reasonable skip ratios between 20.72\% and 83.25\%. Simply applying FixThreshold works well already, Three-stage achieves better accuracies. It achieves 0.89\%--4.13\% accuracy improvement over all four datasets. We can safely draw the conclusion that loss threshold is effective, and our method achieves much higher accuracy under the same skip ratio.
% However, When skip ratio is between 98.91\% and 99.81, loss threshold has less accuracy than random skipping. 
% \xzlNote{maybe not talk about threshold=0.7}
% These are extremely large skip ratio which provides very limited information for training the model. We suspect the reason is (1) there are very few data instances left to train the model. (2) the left data instances have very high loss, which means they won't benefit classifying the majority of data.- But random skipping will find more general data after all.

\paragraph{Efficacy of automatic threshold}
%Since we can find comparable performance with loss threshold. The next question is how to automatically find a desirable threshold to get rid of sweeping? 
\textit{AutoThreshold} can find a loss threshold that results in competitive accuracy and efficiency. 
\autoref{tab:e2e-combined} compares \textit{AutoThreshold} to \textit{FixedThreshold}, showing that  
the former delivers higher AGOT than all the fixed thresholds tested; 
in fact, it delivers \textit{both} higher accuracy and lower training time than most of the fixed thresholds. 



%The former delivers higher accuracy and lower training time  
%is able to find quite similar loss threshold as one of FixThreshold. Among all four datasets, AutoThreshold results have greater accuracy-efficiency than FixedThresholds's. In SST2 and AMZ, AutoThreshold have close threshold to 0.5 (0.51 and 0.52 respectively). They achieve both higher accuracy and less run time with fix threshold = 0.5, which
%achieves higher AGOT. In QNLI and QQP, the automatic threshold is close to 0.7 (0.69 and 0.68 respectively) and they achieve accuracy comparable with fix threshold = 0.5 via runtime between fix threshold = 0.5 and 0.7. However, FixThreshold has very low accuracy and run time on these two datasets.

\paragraph{Efficacy of the meta predictor}
The meta predictor is essential to our efficiency as it skips a large fraction of forward passes, as shown in \autoref{tab:e2e-combined}. 
Compared to \textit{AutoThreshold} which can only skip backward passes, 
our Three-stage training reduces the training time by \textit{additional} 2.01$\times$ on average across all benchmarks.
% \xzlNote{what is 0.19? we should use times $\times$,}
% then average across all benchmarks
% \xzlNote{more than 2x saving on SST2 and AMZ?? also summarize others}.
Furthermore, the accuracy is higher by 0.57\% on average, which is likely because the meta predictor better learns training data importance as the training proceeds. By our design, the data filtered by the loss threshold and meta predictor should be highly overlapped, which is shown that up to 70\% of the filtered data overlapped.



% three-stage's training time is reduced significantly, which is the lowest on all benchmarks. Compared with AutoThreshold, there is more than 2x saving on SST2 and AMZ. Meanwhile, three-stage is able to get higher accuracy than AutoThreshold on SST2, QNLI, and QQP. On AMZ, three-stage's accuracy is slightly lower (0.34\%), we suspect it's because the forward and backward pass skip ratio are higher than AutoThreshold. As shown in \autoref{tab:skipratio}, we can understand where the benefit come from. Because three-stage is able to skip a large fraction of forward passes in addition to the backward pass. For instance, skipping-both's saving is 1.48x more than that of skipping backward pass only on QNLI.



\vspace{-1mm}
\subsection{Sensitivity to hyperparameters}
\label{hyperparameters}
\autoref{tab:hyperparam} summarizes our hyperparameters.
We next study their impact on SST2 performance and their reasonable ranges. 

% to which our method shows low to moderate sensitivity, as will be described below. 

%In order to find the best performance we can achieve, we do hyperparameter tuning. Our hyperparameter search yields comparable accuracy and substantial computation reduction.

%As shown in the Table 4, we have 4 hyperparameters: 
% \xzlNote{move the following to sensitivity analysis..}
\paragraph{Number of epochs ($N_{epoch}$)}
% Msgs: (1) as TrainAll, our method gain additional accuracy as more epochs (??); 
% (2) our method sees increasingly high efficiency as more epochs ... why?? we only have stage 2 for 1+ epochs. high efficiency...
As shown in \autoref{tab:epochs}, our efficiency will be more pronounced as $N_{epoch}$ increases. 
Overall, the first epoch gains most of the model accuracy; 
additional epochs yield diminishing return or even fluctuation. 
This is consistent with prior observations \cite{sanh2019distilbert,jiao2019tinybert} and is the reason why users commonly finetune an NLP model for no more than several epochs.
As $N_{epoch}$ increases, our method has similar accuracy (within $\pm 0.6\%$) as \textit{TrainAll} while seeing increasingly higher reduction in the training time,  e.g. 2.36$\times$ when $N_{epoch}$ = 1 and 6.53$\times$ when $N_{epoch}$ = 5. 
This is because only in the first epoch our method runs stage 0 and 1, paying the learning cost; in subsequent epochs, our method remains in stage 2,  invoking the meta predictor to skip most of the forward and backward passes. 
% our meta predictor effectively skips both forward and backward passes; it no longer pays for the learning cost as in the first epoch.


% \xzlNote{Try convert Figure 4 to a table (see epochs.dox). Also revise the caption}

% Additionally, ours is able to save much more when trained for more epochs. For example, ours have 72\% run time saving on SST2 and AMZ when it trains for 1 epoch. Meanwhile, training 2 epochs has total 2.36x run time saving than training 1 epoch, training 5 epochs has even 6.53x run time saving. Ours also has comparable accuracy or marginal accuracy gain when it trains longer across all the benchmarks as shown in \autoref{fig:epochs}. Same as TrainAll, our method gain additional accuracy as training more epochs. For epoch = 1, 2, and 3, our methods has higher accuracy on SST2 with 72\% to 86\% skip ratio. Then accuracies fluctuate when trained for more epochs. Our method's accuracy is slightly lower than vanilla when it's trained for 4 and 5 epochs. However, we manage to achieve only 0.57\% and 0.45\% accuracy drop with 92\% and 88\% skip ratio. We suspect the predictor only updates on data that it believes worth training which makes it overfitting on certain data points. All the statistics are picked with highest AGOT, which means they have the the best accuracy-efficiency trade-off.

% \xzlNote{Xu: revise the remainder of S4.4. We no longer have tables for them. Be concise. }

\paragraph{Number of mini-batches ($N_0$)} 
The fraction of data examples in stage 0. We try fraction of 10\% -- 40\%. In this stage, the model does forward and backward passes on all the data.
% \input{tab-ablation-#stage0}

% \xzlNote{compress}
Accuracies are stable with the increase of $N_0$. From 10\% -- 40\%, average accuracy is 89.68\% $\pm$ 0.35\%.
% 89.30\%, 89.89\%, 89.39\%, and 90.15\%. $N_0$ = 10\% and 30\% have slightly lower accuracies than $N_0$ = 20\% and 40\% by 0.59\% and 0.76\%. 
But normalized run time grows along with $N_0$. $N_0$ = 40\% has 1.95$\times$ longer runtime than $N_0$ = 10\%.
Experiment results show AGOTs are not sensitive to $N_0$, as the differences among them are very small.
% The average AGOT differences among different $N_0$ are between 0.09--2.5.
$N_0$ = 30\% has the lowest AGOT because of lowest accuracy, however $N_0$ = 40\%'s highest accuracy compensates its longest run time. 
When Sliding window size ($W$) and Average loss threshold ($ALT$) = (8 or 16,  0.1 or 0.2), training will not reach stage 2.
% and Average loss threshold ($ALT$) = 0.1 or 0.2, 
% training will not reach the last stage, so does $W$ = 8 and $ALT$ = 0.1, no matter what $N_0$ is. 
% This means the meta predictor will not start working under such harsh stage-transition condition as the average loss is not small enough. 
This because it's hard for the meta predictor to be trained as well as required by these harsh conditions. But it also proves $N_0$ is not a hyperparameter controlling filtering.

\paragraph{Sliding window size ($W$)} 
% \note[YJ]{Please make sure the notations are consistent. For example, in one of the previous section, we use $K$ as the sliding window size}
The sliding window size in stage 1 for collecting predictor losses. The stage transition is determined by the average loss in this window.
% \input{tab-ablation-windowsize}

% \xzlNote{compress}
From the results, both accuracies and normalized run time grow with $W$. The average accuracy for $W$ = $[4, 8, 16]$ is 89.74\% $\pm$ 0.29\%
% are $[89.37\%, 89.79\%, 90.07\%]$ 
and average run time is reduced by 4.77$\times$ $\pm$ 0.64\%.
% 5.56$\times$, 4.76$\times$, and 4.00$\times$. 
Based on this trend, average AGOTs are very stable. The highest AGOT difference ratio is only 0.11\%. The training time increment is because a larger $W$ has higher demand on the meta predictor and it takes longer time in stage 1 and shorter time in stage 2. 
When $W$ and $ALT$ = (8 or 16, 0.1 or 0.2), training will not switch from stage 1 to stage 2.
% When $W$ = 16 and $ALT$ = 0.1 or 0.2, 
% training will not switch from stage 1 to the last stage, so does $W$ = 8 and $ALT$ = 0.1. 
We can find that the switching likely fails under bigger $W$ and lower $ALT$, because they are more difficult condition to fulfill. So $W$ actually controls data filtering.

\paragraph{Average loss threshold ($ALT$)}
The average loss threshold in stage 1 measuring whether the predictor has been well trained. As long as the average loss in $W$ is lower than $ALT$, training switches to stage 2.
% \input{tab-ablation-threshold}

With the increment of $ALT$, accuracies decrease. The average accuracy of $ALT$ = $[0.1, 0.2, 0.3, 0.4, 0.5]$ is 89.37\% $\pm$ 0.36\%,
% are $[89.74\%, 89.68\%, 89.56\%, 89.02\%, 88.85\%]$, 
their differences are between 0.06\% -- 0.89\%. The normalized run time decreases with $ALT$ from 4.39$\times$ to 6.49$\times$ of \textit{TrainAll}'s run time. Average AGOTs are also stable, its maximum difference is only 1.2\%. 
Similar with $W$, $ALT$ controls whether training goes to the last stage or how much filtering we do.
% When $W$ and $ALT$ are very small, training will continue without querying the meta predictor. 

\input{tab-freeze}
\vspace{-2mm}
\subsection{Compatibility with layer freezing (LF)}
\vspace{-1mm}
Our method complements LF (i.e. training only last few layers), a common optimization for finetuning~\cite{sun2019fine,lee2019would} . 
Table~\ref{tab:freeze} compares \textit{TrainAll} and our method both freezing all but the last layer. 
First, our method is compatible with LF. 
Compared to \textit{TrainAll} with LF, our method with LF achieves comparable accuracy (lower by 0.46\% -- 1.61\%) in much lower training time (lower by 1.75$\times$ -- 7.14$\times$). 
% \xzlNote{use times}). 
Second, our method is still relevant when LF is in use: applying LF to \textit{TrainAll} reduces the training time by 2.34$\times$ with accuracy loss of 2.88\% on average; 
by comparison, our method can reduce additional 2.78$\times$ lower training time at 3.29\% accuracy loss. 
The results encourage use of our method and LF in conjunction. 

% \xzlNote{Table 7: update caption. }

% We also apply our method on vanilla model with well known optimization techniques. The results in Table 11 turns out our method works with layer freezing really well. We show our method's significant benefit of both accuracy and efficiency even with layer freezing. Ours save lots of run time across all four datasets. For example, AMZ needs only 14\% run time and SST2 takes 21\% run time. For accuracy, our method+freezing achieves comparable accuracies with TrainAll+freezing. SST2 has the smallest accuracy gap of 0.46\% and the largest accuracy gap is from QQP which is 1.61\%. This proves that our method is orthogonal and compatible with layer freezing.




==> CamRd_IJCAI_efficient_NLP_Latex/fig-overview.tex <==
% !TeX root = main.tex
\begin{figure}[t]
	%	\centering
	\includegraphics[width=0.48\textwidth]{./figs/highlight-res1}
	%	\vspace*{-2em}
	\caption{Our method significantly reduces training time (columns, right y-axis) while achieving accuracies (lines, left y-axis) comparable to training with all the data. Benchmark details in \nameref{sec:eval}.
	GPU: Nvidia RTX 2080Ti.}
	\label{fig:highlight-res}
	%	\vspace{-5mm}
\end{figure}



==> CamRd_IJCAI_efficient_NLP_Latex/fig-pareto.tex <==
% !TeX root = main.tex

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{./figs/pareto6.pdf}
		\vspace*{-2mm}
	\caption{Compared to training with all data, our method achieves comparable accuracy in a much shorter training time (i.e. higher efficiency). Each plot shows multiple results of our method, resulted from different hyperparameters. 
%	The Pareto from which ones on the Pareto front are highlighted. Best AGOT one prefers accuracy but consider run time if it's much lower.
% 	\textbf{XXXX discuss below} We only plot hypermarameters which achieve accuracy $\pm1\%$ of vanilla performance.
	}
	\label{fig:pareto}
		% \vspace{-5mm}
\end{figure*}



==> CamRd_IJCAI_efficient_NLP_Latex/fig-workflow.tex <==
% !TeX root = main.tex

\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figs/workflow}
% \caption{An overview of the algorithm, showing how training data flows in three stages}
\caption{An overview of our three-stage training algorithm}
\label{fig:workflow}
\vspace{-3mm}
\end{figure}

==> CamRd_IJCAI_efficient_NLP_Latex/header.tex <==

% !TeX root = main.tex

%
%\usepackage{epsf,epsfig,textcomp,amsmath,amssymb,subfigure,cite,moreverb}

%\usepackage[table,xcdraw,dvipsnames]{xcolor} % xzl: if want to use auto gen table from  http://www.tablesgenerator.com

\usepackage{wrapfig}
\usepackage{comment}
%\usepackage{array}
\usepackage{colortbl}

% \usepackage{hyperref}
\def\UrlBreaks{\do\/\do-}

%\usepackage[T1,hyphens]{url}
%\usepackage[colorlinks,urlcolor=blue]{hyperref}
%\usepackage{url}

%\usepackage{MnSymbol} % star symbols, etc
\usepackage{amsthm} % unnumbered theorem etc

%\usepackage{times}
\usepackage{color,soul}
%\usepackage{soul}
%\usepackage{xcolor}
\usepackage{graphics}
\usepackage[hidelinks]{hyperref}
\usepackage{lipsum}
\usepackage{tikz}
\usepackage{enumitem}	% for fine control of list env
\usepackage{listings} % for code listing
%
\usepackage{booktabs}	% xzl: for fancy tables
\usepackage{lipsum}

\usepackage{capt-of}	% xzl: used to override the ``figure'' and ``table'' in caption.

\usepackage{todonotes}  %xzl: for "missing figures"
\usepackage{subcaption} %xzl: for subfigure. incompatible with package subfig

% \usepackage[color]{showkeys}	 % xzl: comment this out in final draft
% \definecolor{refkey}{rgb}{249,158,26}
% \definecolor{labelkey}{rgb}{0,1,0}

%\definecolor{labelkey}{rgb}{0,0,1}
%\definecolor{refkey}{rgb}{0,0,1}

% --- all sorts of math fonts ---
% cf: https://tex.stackexchange.com/questions/58098/what-are-all-the-font-styles-i-can-use-in-math-mode
\usepackage{mathrsfs}	% xzl: for Ralph Smith’s Formal Script Font (rsfs)
\usepackage{amsfonts}
%\usepackage{inconsolata} % xzl: this uses inconsolata for texttt

\usepackage[export]{adjustbox} % xzl: flush figure to left/right

\usepackage{algorithm,algorithmic,amsmath} % jin: for pseudo code
\usepackage{boldline}					% jin: use boldline in the table

\usepackage{multirow}


\newtheorem*{thm}{Theorem}
% -- diff styles --- 
% \newtheorem{definition}{Definition}[section]
\newtheorem*{definition}{Definition}
\newtheorem*{assumption}{Assumption}

%\usepackage[dvipsnames]{xcolor}

%
%%\usepackage[bookmarks, breaklinks=true, colorlinks=true, plainpages = false,
%%  citecolor = blue, urlcolor = blue, filecolor = blue,]{hyperref}
%
%\usepackage[labelfont=bf,font=medium]{caption}
%\usepackage[labelfont=bf,textfont=normalfont]{caption}
%\usepackage{multirow}
%
%\renewcommand\section{\@startsection {section}{1}{\z@}%
%   {-3ex \@plus -1ex \@minus -.2ex}%
%   {1.7ex \@plus.2ex}%
%   {\normalfont\large\bfseries}}
%\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%   {-2ex\@plus -1ex \@minus -.2ex}% used to be -2.5
%   {1ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%\renewcommand\subsubsection{\@startsection{subsubsection}{2}{\z@}%
%   {-1ex\@plus -1ex \@minus -.2ex}%
%   {0.3ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%
%\newcommand\minisection{\@startsection{subsubsection}{4}{\z@}%
%   {1ex\@plus 0ex \@minus 0ex}%
%   {-1.5ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%

% ----------- drawing --------------
\definecolor{frenzyorange}{RGB}{249, 158, 26}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,fill=frenzyorange,draw,text=white,inner sep=1pt] (char) {#1};}}
		
%%------------Formatting----------
% nb: \paragraph{} is built-in and will affect many things --- 
\newcommand{\Paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	 % used to be 6pt
%\newcommand\paratitle[1]{\textit{\textbf{#1}}}
\newcommand\paratitle[1]{\textit{\textbf{#1}} \hspace{1mm}}
%\newcommand{\Paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	
%\newcommand\itno[1]{({\em #1})}
%\newcommand\itemno[1]{({\em #1})}

% @paragraph seems built-in. 
\renewcommand{\paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	 % used to be 6pt

%%%%%%%%%%%%%%%% smitemize %%%%%%%%%%%%%%%%%%%%
%
\newenvironment{smitemize}%
  {\begin{list}{$\bullet$}%
     {\setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{2pt}}}%
  {\end{list}}
%
%%%%%%%%%%%%%%%% custom spacing %%%%%%%%%%%%%%%%%%%%
%
%----------- Comments-----------------
\newcommand\Note[1]{\sethlcolor{red} \hl{#1}} % highlighted notes of other colors.
						 % For colors info from xcolor package, check out:
						 % http://en.wikibooks.org/wiki/LaTeX/Colors
\newcommand\Noted[1]{} % remove highlights.

\newcommand\xzlNote[1]{\sethlcolor{yellow} \hl{#1}} % highlighted notes of other colors.

\definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
\definecolor{mygreen}{HTML}{ADFF2F}
\definecolor{mylightgray}{gray}{0.8}
%\newcommand\jin[1]{\sethlcolor{mygreen} {\color{darkblue}\bf\hl{#1}}}
%\newcommand\jin[1]{\fcolorbox{blue}{white}{\bf\em\color{blue}jin:} {\small\em\color{blue}{\fontfamily{qhv}\selectfont #1}}}
\newcommand\jin[2][]{
	\fcolorbox{blue}{white}{\bf\em\color{blue}jin:}
	{\small\em\color{blue}{\fontfamily{qhv}\selectfont \underline{#1} #2}}
}


\newcommand\myfootnote[1]{\textcolor{red}{\footnote{#1}}}

%\renewcommand\thefootnote{\textcolor{red}{\arabic{footnote}}}

%====== for estimating final pages ===== %

% xzl: the one uses package enumitem that can fine tune indent.
% 
% for simplicity, can also use \begin{itemize}[leftmargin=*]
\newenvironment{myitemize}%
  {\begin{itemize}
	[leftmargin=0cm,
		itemindent=.3cm,
		labelwidth=\itemindent,
		labelsep=0pt,
		parsep=1pt,
		topsep=1pt,
		itemsep=1pt,
		align=left]
  }%
  {\end{itemize}}    

\newenvironment{myenumerate}%
  {\begin{enumerate}
	[leftmargin=.cm,itemindent=.5cm,labelwidth=\itemindent,
		labelsep=0pt,
		parsep=1pt,
		topsep=1pt,
		itemsep=3pt,
		align=left]
  }%
  {\end{enumerate}}    

%====== shortcut for ref ===== %
\newcommand\sect[1]{Section~\ref{sec:#1}}	% NB: does not play well with \note{}        

% -------------------FONTS-------------------
%\newcommand{\scenario}[1]{\textit{#1}}
\newcommand{\scenario}[1]{\texttt{#1}}

%\newcommand{\state}[1]{\textsc{#1}}
%\newcommand{\state}[1]{\texttt{#1}}

\newcommand{\system}[1]{\textsf{#1}}

% texttt will be larger than body text..
\newcommand{\code}[1]{\texttt{\small{#1}}}	
%\newcommand{\code}[1]{\texttt{#1}}	

\newcommand{\queue}[1]{\textit{#1}}
% ----------------------------------------------

%--------------------------------------------------------

\input{terms}

% Remove the copyright block space.
% http://ryanlei.wordpress.com/2012/02/13/latex-remove-the-copyright-space-from-the-acms-sig-alternate-template/
\makeatletter
\def\@copyrightspace{\relax}%
\makeatother


==> CamRd_IJCAI_efficient_NLP_Latex/intro.tex <==
% !TeX root = main.tex

\section{Introduction}
\vspace{-1mm}
%\xzlNote{need an intro figure?? -- can be a highlight of our result}\note[YJ]{I usually prefer to have a figure that summarizes the basic idea in the introduction section}

\paragraph{Efficient model finetuning}
Modern NLP models are pretrained on large corpora once and then finetuned for specific domains. % downstream tasks. 
Efficient finetuning is crucial because 
(1) as opposed to one-off pretraining, 
finetuning is invoked for every downstream task and even on individual user's data \cite{houlsby2019parameter}; 
(2) finetuning is often performed close to where the domain training examples reside, e.g. smartphones \cite{rebuffi2018efficient}; 
these platforms often have constrained computing resources. 
As NLP models become larger \cite{devlin2018bert} and language tasks diversify, it is compelling to finetune a model with fewer resources without comprising accuracy much~\cite{zaken2021bitfit,jiang2019smart}.  

% Modern NLP models are pretrained on large corpora once and then finetuned for specific domains. % downstream tasks. 
% Efficient finetuning is crucial because 
% (1) as opposed to one-off pretraining, 
% finetuning is invoked for every downstream task and even on individual user's data \cite{houlsby2019parameter,pmlr-v97-stickland19a,peng2019transfer,qiu2020pre}; 
% (2) finetuning is often performed close to where the domain training examples reside, e.g. smartphones \cite{rebuffi2018efficient,sanh2019distilbert,jiao2019tinybert,sun2020mobilebert}; 
% these platforms often have constrained computing resources. 
% As NLP models become larger \cite{devlin2018bert,brown2020language,radford2019language,liu2019roberta} and language tasks diversify, it is compelling to finetune a model with fewer resources without comprising accuracy much~\cite{zaken2021bitfit,jiang2019smart}. 




%\note[YJ]{while talking about prior work, we should highlight the limitations or something missing from prior work}

% Much machine learning work focuses on improving accuracy. Yet, accuracy-efficiency trade-offs are nevertheless appropriate given constrained resources. This is particularly true for fine-tuning, which is performed where the domain data resides. 
Importantly, prior work also has recognized the importance of efficient finetuning. 
% to reduce training resource consumption (e.g. GPU time) while achieving similar accuracy.  
A popular approach is to impose efficient model structures~\cite{sun2019fine}, including low rank approximation \cite{lan2019albert,ma2019tensorized}, weight sharing \cite{dehghani2018universal,lan2019albert}, knowledge distillation \cite{hinton2015distilling}, pruning \cite{cui2019fine,mccarley2019structured}, quantization \cite{jacob2018quantization}, and layer freezing \cite{lee2019would}.
%\note[YJ]{we may need to be specific about what value of our proposed work, for example, a or some remaining issues that prior works ignore or cannot address} 
% \change[YJ]{This}{While most of work focuses on modeling strategies, this}


While most of the work focuses on modeling strategies, this paper exploits an opportunity particularly for finetuning with large datasets:
% \add[YJ]{particularly when fine-tuning with large datasets}: 
%\textit{efficient use of training data} \textbf{fast training through low-cost data down-selection... (or filtering....??)}. 
\textit{filtering training data at low computational cost}. 
Given that training data is known as often redundant \cite{katharopoulos2018not},
we test a simple idea: skip training examples that are less important to the gradient updates. 
% \change[YJ]{the training accuracy.}{gradient updates.}

%\input{fig-overview}
\input{tab-overview}

\paragraph{Challenges}
The idea raises twofold challenges. 
% \remove[YJ]{First, how to identify training examples}
First, how to assess training example importance? 
As the model is being updated throughout a training process, 
the assessment must weigh training examples against the model's \textit{up-to-date} capability. 
Second and more importantly, 
the assessment itself should incur low computational overhead. 
To this end, much prior work for selecting training data does not apply \cite{mirzasoleiman2020coresets,wang2020optimizing}: 
targeting training effectiveness but not efficiency, they often use computationally expensive methods to weigh data, e.g. comparing training gradients; 
they often slow down training or incur costly prepossessing before training. 

%pror work on data selection: (the reason why we do not cmp vs prior data selection and data weihgting).. 
%their goal: effectiveness; therefore pay the cost of trianig anyway. but make good use of the training results (e.g. graidents, ...) 
%without training with the data. 
%Existing techniques such as gradient comparison does not apply due to their high cost.\note[YJ]{citation} 

%finetuning often finishes after one epoch \xzlNote{cite},\note[YJ]{not sure we should mention this "one epoch" statement, it may raise some questions from reviewers} 
%where each training example is encountered (observed) once. 
%For each example, the trainer (system??) would need to assess its importance and decide whether training is worthy -- without seeing the whole training set. 

\paragraph{Our method}
We use training loss as the signal for data importance: 
low loss means the model has high confidence in the training examples, which could be skipped to avoid the cost.
%Our observation suggests redundancy in training data: 
%Our observation shows great potential in 
As will be shown in the paper, this simple idea is powerful:  
skipping training data on which losses are lower than a fixed, hand-picked threshold $L_{low}$ can skip 20\% -- 50\% of the data 
% \xzlNote{numbers inconsistent with the abs?} 
while seeing a minor ($<$1\%) drop in the final model accuracy. 
Yet, hand-picking $L_{low}$ is tedious; 
comparing $L_{low}$ against losses still requires the computation of forward passes. 
%This motivates us to design an automatic data filtering algorithm. 

%Loss requires no extra computation beyond a forward pass, 
% As this paper will show, 
%a simplistic strategy -- 
%running forward passes on all minibatches while skipping backward passes for those with losses lower than a fixed, hand-picked threshold $L_{low}$, 
%skipping backward passes for minibatches with losses lower than a fixed, hand-picked threshold $L_{low}$, 

%\note[YJ]{Some of the following parts contain technical details and can be moved to the method section}

%To fulfill the efficiency potential and minimize manual efforts, 
To this end, we propose an algorithm that learns to
predict data filtering decisions in tandem with training. 
Given a model and training data, the algorithm automatically derives a proper loss threshold $L_{low}$ and further skips forward and/or backward passes on training data, whenever appropriate.
%predict filtering (skipping) decisions without computing losses. 

The algorithm runs training as a multistage process: each stage receives supervision from earlier stages but is more efficient than the former. 
After training starts: 
% \note[YJ]{Should we use the same itemize format?}
%The algorithm comprises three stages, each is 
%The trainer integrates the above two techniques in a three-stage process. 
\begin{myitemize}
\item 
%(1) 
The first stage derives $L_{low}$ that adapts to the model and the training data. 
This stage runs both forward and backward passes on training examples. 

\item 
The second stage uses the derived $L_{low}$ to filter backward passes.
%It runs forward passes on all examples while using $L_{low}$ 
With the filtering decisions, it trains a meta predictor based on simple linguistic features
of input texts. This meta predictor will later decide if the given examples are worth training.

\item 
The third stage queries the meta predictor to filter both forward and backward passes. 
\end{myitemize}

% \xzlNote{the following two sentences unclear. revise.}
% When training a predictor to do filtering, our predictor loss here is the negative log likelihood. As long as the predictor loss is sufficiently low, we reply on the predictor to do data skipping.
%It continues to train the predictor. 
%and trains a naive Bayesian classifier. 
The first two stages are short (processing average 16.1\% of
% \xzlNote{XXX} 
examples across all benchmarks) while the most efficient third stage processes most examples.
The algorithm automatically advances across the stages, based on its observation of training losses and the meta predictor's performance. 

\begin{comment}   %--- too detailed ---%
(1) 
\textit{automatic loss thresholds.}
%The trainer removes the need for a hand-picked $L_{low}$ and instead determines $L_{low}$ adaptively. 
The trainer derives $L_{low}$ . 
To do so, it sets $L_{low}$ as the moving average of the losses in a sliding window. 
The rationale is \xzlNote{...}
Our experiments show that such an adaptive $L_{low}$ quickly converges close to the hand-picked optimal value, and is robust to the initial value of $L_{low}$. 
As a result, the trainer skips backward passes for any minibatches with losses lower than $L_{low}$. 

(2) 
\textit{The loss predictor.}
To further skip forward passes for less important examples, 
the trainer learns to predict the losses of examples -- without executing a forward pass to get their losses
To do so, it runs a naive Bayesian classifier which takes as input the word frequencies of a training sentence and predicts if the loss will exceed $L_{low}$. 
This design is motivated by extensive linguistic evidence \xzlNote{...}
Accordingly, the trainer runs forward pass only on training examples that the classifier predicts worthy ($L>L_{low}$), and skip the examples otherwise. 
It is worth noting that the trainer does not pre-train the classifier; 
instead, for each fine-tuning task it trains a classifier from scratch, in conjunction to the training of the NLP model. 
\end{comment} 


\paragraph{Results}
On a diverse set of NLP benchmarks, 
% {\color{blue} we present competitive trade-offs. Our accuracy decrease is too minor to matter ($<$1.4\%); on some datasets, we even \textit{gain} accuracy. Meanwhile, our efficiency gain is very significant (5$\times$). }
our algorithm reduces the total training time by up to 6.7$\times$ (5.88$\times$ on average). 
The resultant accuracy degradation is minor, no more than 1.44\% (0.6\% on average). 
An ablation study shows the efficacy of our techniques: 
(1) the automatic loss threshold skips backward passes for up to 84\% of the training examples; % reducing the total training time by 2x; 
%compared to a set of fixed thresholds, it reduces the training delay by up to 39.69\%;
%compared to optimal thresholds from exhaustive search, it only has delays difference of 4.16\% in average. 
(2) the meta predictor skips forward passes for up to 81\% training examples when trained for 2 epochs;
% \xzlNote{why do we mention both 1 and 2 epochs}
% (44.29\% and 67.37\% on average), 
% which reduces total training delay by 21.80\% and 38.37\% atop the adaptive threshold. 
% (3) 
% \xzlNote{the point still valid?}
% the training process finds splits between stages close to optimal, with training delays up to 61.54\% lower as compared to exhaustive search. 
(3) as the number of epochs grows, our efficiency is increasingly higher, e.g. up to 18.1$\times$ training time reduction with 1.83\% lower accuracy when training for 5 epochs on SST2 \cite{wang2019glue}.
% \xzlNote{what does ``on one benchmark'' mean}

% --- Xu's --- 
\begin{comment}
our algorithm reduces the training delay by up to 85.19\% (73.05\% on average with 2 epochs). 
The resultant accuracy degradation is minor, no more than 1.02\% (0.45\% on average). 
An ablation study shows efficacy of our techniques: 
(1) the adaptive loss threshold skips backward passes for up to 83.87\% training examples (a 56.73\% reduction in total training delay); 
compared to a set of static thresholds, it reduces the training delay by up to 39.69\%;
compared to optimal thresholds from exhaustive search, it only has delays difference of 4.16\% in average. 
(2) the loss predictor skips forward passes for up to 58.56\% and 81.01\% training examples for training for 1 and 2 epochs respectfully (44.29\% and 67.37\% on average), which reduces total training delay by 21.80\% and 38.37\% atop the adaptive threshold. 
(3) the training process finds splits between stages close to optimal, with training delays up to 61.54\% lower as compared to exhaustive search. 
\end{comment}

\paragraph{Contributions}
\begin{myitemize}
\item 
%(1) 
We presented empirical evidence that large NLP datasets
are redundant for model finetuning, and many training examples can be filtered with a low impact on accuracy. 

\item 
We proposed a simple, automatic mechanism for filtering training data:
using an automatic loss threshold for skipping backward passes and a lightweight meta predictor for further skipping forward passes.

\item 
We presented a holistic training process that integrates the above techniques and demonstrated its efficacy on diverse NLP text classification tasks. 

\item
We proposed a novel, comprehensive evaluation strategy: using a new metric considering both the accuracy and efficiency; estimating the energy consumption to reduce CO$_2$ emission.
\end{myitemize}
% \note[YJ]{Should we also talk about the evaluation strategies? For example, AGOT and the estimation on energy consumption, which to my understanding are novel in NLP/ML works on efficient training.}

==> CamRd_IJCAI_efficient_NLP_Latex/method.tex <==
\section{Our Method}
%Our overall approach is to use training loss for filtering training data. 
Let us assume that the whole training set is divided into $M$ mini batches $\mathcal{D}=\{D_m\}_{m=1}^M$ and each mini batch consists of $N$ training examples.
The training loss for the $m$-th mini batch is defined as:
\vspace{-1mm}
\begin{equation}
\label{eq:loss}
  l(m) = \frac{1}{N}\sum_{n=1}^{N}CrossEntropy(\hat{y}^m_n, y^m_n)
\end{equation}
where $\hat{y}^m_n$ is the model prediction and $y^m_n$ is the ground truth.
Intuitively, if the model is confident with all the examples in this mini batch, we should expect that the average loss $l(m)$ will be very small, and skipping the training on this mini batch would not cause a big difference in model performance. The strategy of skipping individual examples allows for a more granular level of impact control.
Furthermore, we hypothesize that, for a given input sentence, the words in the sentence may provide enough clues about the model's confidence level.
For example, if the model gives high confidence prediction on a group of words, we should expect it to show high confidence in sentences having the same words.

%We design a training algorithm by answering a set of questions: 
We address the following design questions: 
\begin{myitemize}
% \item How to skip the backward pass of a mini batch \emph{with} its training loss? 
%\item How to selectively skip backward passes on mini batches given their training loss? 
\item How to select mini batches and skip their backward passes, given their training loss? 
%\item Furthermore, how to skip a mini batch \textit{without} calculating its training loss, which will further eliminate the forward computation on the data?
%forward passes which calculate the training loss; 
%\item Furthermore, how to selectively skip forward passes on mini batches \textit{without} calculating training losses?
\item Furthermore, how to select mini batches and skip their forward passes, 
\textit{without} calculating their training losses?
% hence further eliminating the forward computation on the data?
\item How to realize the two above mechanisms in an efficient, automatic manner?
\end{myitemize}



\vspace{-1mm}
\subsection{Three-stage training}
\label{3stages}
\begin{comment}
\begin{table}
\centering
{\small
  \begin{tabular}{lccc}
    \toprule
    & Stage 0 & Stage 1 & Stage 2\\
    \midrule
    \emph{Neural classifier}\\
    Forward & \cmark & \cmark & \faFilter\\
    Backward & \cmark & \faFilter & \faFilter \\
    \midrule
    Meta predictor & - & Training & Prediction\\
    \bottomrule
  \end{tabular}
  }
  \caption{\label{tab:three-stage} The computational cost of the proposed three-stage training algorithm. \cmark indicates that the operation is mandatory, while \faFilter means it's optional. The bottom row of this table shows the actions on the meta predictor.}
\end{table}
\end{comment}

\input{fig-workflow}

Our proposed algorithm consists of three consecutive stages; 
the dataflow of each stage is shown in Figure~\ref{fig:workflow}.
Throughout the process: stage 0 warms up training and estimates a loss threshold for selecting mini batches; 
stage 1 filters out mini batches by referring to the estimated threshold, meanwhile using the filtering results to train a meta predictor; 
stage 2 uses the meta predictor to filter out mini batches without explicitly calculating their forward losses. 
Each stage requires supervision in earlier stages to become effective but is more efficient than the former. % as illustrated in \autoref{tab:three-stage}.
%The rest of this section will explain the three stages in detail.

\paragraph{Stage 0: estimating loss threshold}
This stage warms up the model training and automatically derives the loss threshold $L_{low}$.
For each mini batch, the algorithm runs both the forward step for computing the training loss and the backward step for gradient update. 
After training with the initial several mini batches, the loss threshold is estimated by the moving average of recent training losses:
\vspace{-1mm}
\begin{equation}
 L_{low}(m) = \frac{1}{K}\sum_{k=1}^{K} l(m-k)
\end{equation}
where $l(m)$ is the training loss calculated on the $m$-th mini batch defined in \autoref{eq:loss}, and $K$ is the window size of moving average. 
Prior work already used the moving average of training losses to estimate the trend of loss changes and monitor the training process \cite{zhang2019autoassist}.
This work further uses the moving average to identify mini batches worth training, i.e. if the training loss on a mini batch is higher than the moving average. 
% , then it should be used to update the model parameters.
Our study shows that, with a small window ($K=8$), 
% $L_{low}(m)$ 
the loss threshold quickly stabilizes with low variations. 
For instance, the variation becomes less than $4.3\times10^{-5}$ on QNLI when stage 0 spans the first $7.7\%$ of training data. 
% e.g., $m \geq $ first $7.7\%$ training data with variation of $4.3\times10^{-5}$ on QNLI). 

\iffalse
We derive $L_{low}$ automatically from on a small sample of the training data. 
The mechanism is as follows. 
The trainer pre-shuffles all training data randomly. 
As it runs it maintains a sliding window, which consists of losses of most recent $w$ examples. 
The trainer sets $L_{low}$ to be the mean of the sliding window. 
\fi

\paragraph{Stage 1: training the meta predictor}
With a stabilized loss threshold $L_{low}$, the algorithm moves to the first stage of training, in which it can filter out some mini batches if their losses are lower than $L_{low}$. 
To further prepare for stage 2, the algorithm starts to build a meta predictor $f$, which aims to predict the filtering decision for a mini batch \emph{without} resorting to the forward pass.
Specifically, we implement the meta predictor $f$ as a binary naive Bayes classifier:
\begin{equation}
\label{eq:naive-bayes}
f(\vec{w}^m)\in\{0, 1\}
\end{equation}
where $\vec{w}^m$ represents the bag-of-words representations of the input sentences in the $m$-th mini batch; 
the predicted value 1 indicates that the training loss is likely to be higher than the threshold, while 0 indicates that the loss is likely to be lower than the threshold. 
With the forward computation on mini batch $m$ and the loss threshold $L_{low}$, this mini batch provides a training example for updating the meta predictor $f$.

In order to measure how much information the meta predictor learns, 
we use the same notations as above and additionally define $y'$ as the ground truth label, 
which indicates if elements in the mini batch $m$ are worth training by comparing their forward losses with $L_{low}$. 
The meta predictor's loss is defined as: 
% \note[YJ]{I have a question about the technical detail: does the meta predictor (1) give one mini-batch a single label or (2) assign each sample in the mini-batch an individual label? If it is the second case, how do we know whether we should skip one mini-batch? If it is the first case, then should $y'$ in the following be defined on the mini-batch level?}
\vspace{-1mm}
\begin{equation}
\label{eq:predictorloss}
  l_{mp}(m) = -\frac{1}{N}\sum_{n=1}^{N}\log p({y'}^m_n\mid \vec{w}^m_n)
\end{equation}
If the meta predictor exhibits sufficient low moving average losses, stage 1 ends.

In a nutshell, the meta predictor further saves the computational cost if it deems that the target language model is likely familiar with the examples in a mini batch. 
For this purpose, it is sufficient for the predictor to run Naive Bayes classification on the input words because lexical information is an essential component of a text's semantic information.
The following section on~\autoref{sec:discussion} will present more design choices. 

\iffalse
After $L_{low}$ stabilizes (with sufficiently low variations), the trainer stops updating it. 
It starts filtering training data by comparing their losses to $L_{low}$. 
With such loss-based filtering decisions, the trainer trains a predictor -- a Naive Bayesian classifier of simple linguistic features (BoW). 
The trainer does not query the predictor. 
This stage runs forward passes on all data (in order to get their losses) while selectively running backward passes only on data surviving the filtering.

\xzlNote{Writing below needs work}
Specifically, the predictor works as follows. 
We train a Bernoulli Native Bayesian Classifier (NBC) to pick out data that the model needs to do back-propagation on. 
To train the predictor, we get the labels by running forward passes to get the loss and comparing it to $L\_{low}$. 
To query the predictor, we take an example and feed its BoW features to NBC. 
In case the NBC predicts negative (``no train''), we skip the example with no more computation;
otherwise, we run a forward pass, get the loss, and only run backpropagation if the loss exceeds $L\_{low}$. 
As this loss-based decision is new data for the NBC, 
we update the NBC with it (i.e. continuously train the NBC online)
\fi

\paragraph{Stage 2: filtering data with the meta predictor}
Once the meta predictor shows adequate performance, 
%(as validated by loss-based selection on new data), 
the algorithm queries it for screening each mini-batch. 
On a mini-batch that the predictor deems worth training, the algorithm runs a forward pass and uses the resultant loss to decide if a backward pass is needed. 
% otherwise, the trainer skips the data without a forward or backward pass.
Hence, stage 2 can skips both forward and backward passes for high efficiency.

With our design, the training process reaches stage 2 soon after the first epoch starts, as we will demonstrate in the evaluation.
In case the training spans more than one epoch, the process remains in stage 2 in subsequent epochs. 


\iffalse
We stitch the three stages as follows.
The trainer switches from stage 0 to stage 1 once $L_{low}$ is stable. 
It sets stage 0 to span $n_0$ mini-batches, a hyperparameter we set empirically. 
The trainer switches from stage 1 to stage 2 once the predictor has adequate accuracy: 
as long as the predictor achieves an average lower higher that $L_{trans}$ in a sliding window \xzlNote{what size}. 
We will experimentally evaluate the impact of the two hyperparameters.
\fi

% In terms of training data that makes an impact, our approach has similarities with the Perceptron algorithm, which only updates the model based on the data that it makes mistakes and puts the correctly classified data aside.
\vspace{-1mm}
\subsection{A Special Case}
% Our Three-Stage training will only reach the next stage when former stage ends. Therefore, we updates the loss threshold $L_{low}$ during stage 0 then use it in both stage 1 and stage 2. However, finding comparable accuracies requires extensive hyperparameter tuning. Utilizing $L_{low}$ directly to filter out low-loss data instances could also achieve comparable accuracy and good accuracy-efficiency trade-off (as shown in \autoref{sec:eval}) with no hyperparameter finding at all. We name this filtering method as Automatic-threshold Training. It can be considered as a special case of Three-stage training and it's a easy, straightforward, and ready-to-go method.

% \xzlNote{the following writing downplays our contribution and may backfire; instead, compare to the following version:}

While the three-stage algorithm is effective (as \autoref{sec:eval} will show), it is possible to use a stripped-down version of it: 
after determining $L_{low}$ automatically, use it to filter all the remaining training data without invoking the meta predictor. 
Doing so would miss the opportunity of skipping forward passes; 
yet, by eschewing the meta predictor and its hyperparameter tuning, the method further simplifies training. 
We refer to this method as \textit{automatic threshold only} and will compare to it in \autoref{sec:eval}. 



% \note[YJ]{Not sure I get all the special cases of the proposed algorithm. Will need another discussion for better understanding.}

==> CamRd_IJCAI_efficient_NLP_Latex/related.tex <==
% !TeX root = main.tex

\section{Related Work}
\vspace{-1mm}
%
%\annote[Xu]{}{1. I think APT and Percptron are more close to Data selection in training, but Yangfer suggests we should put these two at the beginning. Can we switch the order of first two paragraphs and still leave these algorithm at the beginning? 2. The three paragraph names look vague, but I don't have better alternatives.}
% \xzlNote{curriculum learning}
\paragraph{Effective training}
Aggressive-passive training (APT) \cite{shalev2003online} and Perceptron \cite{rosenblatt1958perceptron} are well-known online learning algorithms that only update the model either on high-loss or misclassified samples. 
% \st{However, training effectiveness not efficiency are their goals for the design.}
Unlike our method that can skip \textit{both} forward and backward passes, these methods would require forward passes on all the training data, which is much less efficient.
% \xzlNote{However, they ... (how are we diff from APT/perceptron)?}
% Rather than considering all samples having the same performance contribution,
% \annote[YJ]{Rather than considering all samples simultaneously,}{most training algorithms for deep learning cannot consider all the training data simultaneously.} 
%To facilitate learning, the training model could be presented with the training data in a meaningful order. 

Curriculum learning \cite{bengio2009curriculum} trains a model from the easiest examples to the hardest ones, hence accelerating model convergence. 
%and finding better local minima in deep learning methods. 
Yet, arranging the data order requires prior domain knowledge of all training data, e.g. how ``noisy'' are these examples, which can be very expensive to preprocess a large dataset to collect such information.
% \xzlNote{which can be expensive to obtain? why??}
To get rid of this requirement, self-paced learning \cite{NIPS2010_e57c6b95}
updates model weights by considering the level of difficulty of given examples. 
% if an example is easy and an extent weight determining how easy the sample is. 
%By decreasing the extent weight in each iteration, model weights are gradually updated with more difficult data. 
Unlike us, these techniques do not filter training data; 
they incur high optimization costs on large NLP models and datasets.

\paragraph{Training data selection}
Motivated by training data redundancy, previous work downselects the data; 
however, many require expensive data preprocessing, making them expensive for NLP finetuning. 
Importance sampling~\cite{katharopoulos2018not} can train with smaller data batches that have a similar gradient norm as the full data batches. 
CRAIG~\cite{mirzasoleiman2020coresets} selects training examples for which the weighted sum of gradients closely approximates that of the full training set. However, these two methods sample important data by solving the optimization problem for each data to mimic the \textit{full} data gradient. 
% \xzlNote{However, .... they solve the optimization problem for each data to mimic the full data gradient...}
% \st{Not each of them is equally important.} 
% Some data and model components can be removed without hurting or even improving the performance due to the increased model flexibility. 


% \paragraph{Filtering training data with losses.} This is a known idea.
\textbf{Filtering training data with loss} is known. 
Yet, our contributions are (1) a meta predictor for deciding filtering and (2) a multistage process for training the meta predictor. Hence, our proposed training procedure can automatically skip forward and backward computations, a goal unattainable for loss-based filtering. \S\ref{sec:eval} shows that we outperform loss-based filtering.

Our goal is related to active learning but not the same: 
in an unsupervised setting, 
it down-selects unlabeled data for labeling and then training~\cite{settles2009active}. 
However, few active learning methods that employ a multistage process, 
which first trains a meta predictor in a \textit{supervised} fashion and then uses the predictor to filter data in an \textit{unsupervised} fashion. 
To this end, our idea can be extended to support active learning. 

Clustering training data can remove at least 10\% examples for object recognition \cite{birodkar2019semantic}. But it needs to sweep through all the data instances and keep updating clusters before picking out close ones. 
Selection via proxy \cite{coleman2019selection} simplifies the big target model to a small proxy model finding the core-set to train the big target model. Unlike us, the proxy model needs to be trained on all the data samples then they train the target model separately.
% The existing redundancy in training sets motivates us to propose a more data-efficient training mechanism, specifically for NLP.

\begin{comment}   % ---- xzl: not very related ---- 
Reinforcement learning can be used to train a scorer that weights data to benefit learning~\cite{wang2020optimizing}. However, scorer training incurs high overhead and needs an additional development set for testing.
% \xzlNote{what does the following mean? are these data unlabeled? or have noisy labels?}
%Sample selection of noisy labels \cite{xia2021sample} uses data losses to label unlabeled data then collect them to the training set. 
%
% Different from us, they all have lots of computational overhead and most of them are separate from training the target model.
% \annote[YJ]{are data-prepossessing methods.}{not sure how to interpret this statement? Is this a limitation?}
% Importance Sampling \cite{katharopoulos2018not} and CRAIG \cite{mirzasoleiman2020coresets} sample important data by solving the optimization problem for each data to mimic the full data gradient. 
% Clustering \cite{birodkar2019semantic} needs to sweep through all the data instances and keep updating clusters before picking out close ones. 
% Proxy \cite{coleman2019selection} formulates the core-set by keeping data it has low accuracy on. Selection by RL \cite{wang2020optimizing} cares accuracy and noisy labels selection \cite{xia2021sample} has a different task with us.
% However, their methods have significantly lower efficiency.
Compared to them, our goal is to do data selection in parallel with training the target model and take model losses, not gradients, as the metric. Besides, our meta predictor is trained with simple linguistic features (Bag-of-Words),
% \annote[YJ]{not training data instances themselves,}{not sure I understand this line}
ensuring efficient selection. 
% \xzlNote{this is good. But how is our work different? new?}
\end{comment}

% \note[YJ]{I have a question about discussing the related works in the current order: as the previous paragraph concludes the methods mentioned before, does it mean the following two methods do not have significant computational overhead?}
% Data selection by Reinforcement Learning~\cite{wang2020optimizing} uses RL to train a scorer that weights data to maximally benefit learning, which has accuracy given a same training set.
% \xzlNote{increase accuracy from given a training set?}
% But it has lots of computing overhead and they care about finding how much attention the model should pay to different data. 
% \xzlNote{``Their goal is different ... significantly lower efficiency...''}
% Sample selection of noisy labels \cite{xia2021sample} uses data losses to label unlabeled data then collect them to the training set. 
% However, their goals are different from us and their methods have significantly lower efficiency.
% But we are working on tasks that have clear labels instead of updating the model with labels more likely to be correct. \xzlNote{any connection at all? e.g. do they filter training data?}
% \xzlNote{what's our benefit vs them?}

AutoAssist~\cite{zhang2019autoassist} shares our motivation: to filter  training data with a small model called ``assistant''. 
% Although AutoAssist was shown to reduce the \textit{training loss} at a higher rate, it was unclear by how much it can reduce the \textit{training time} without degrading accuracy much. 
Although the paper shows that AutoAssist reduces the \textit{training loss} at a higher rate, it was unclear by how much \textit{training time} is reduced. 
The assistant is complex, e.g. stochastic sampling data to generate a batch, which takes more than ten epochs to warm up, unsuitable to NLP finetuning which comprises no more than several epochs.
By contrast, our design is simple, saving training time significantly even for one epoch. The saving is increasingly higher as the epoch count grows. 
We will experimentally compare to AutoAssit in \S\ref{sec:eval}.
%the first several epochs see similar or even lower efficiency compared to training with all data~\cite{zhang2019autoassist-arxiv}. 
%As such, AutoAssist is suitable to model pretraining comprising tens or hundreds of epochs but not finetuning which lasts no more than several epochs. 

%Compared to our design, the assistant is more complex, e.g. sampling data in a stochastic fashion and asynchronous update, which takes more than ten epochs to warm up; 
%the first several epochs see similar or even lower efficiency compared to training with all data~\cite{zhang2019autoassist-arxiv}. 
%As such, AutoAssist is suitable to model pretraining comprising tens or hundreds of epochs but not finetuning which lasts no more than several epochs. 
%\xzlNote{our algorithm is simpler -- do not have to sample to construct a minibatch}
%\begin{itemize}
%\item No training accuracy (only training loss) was reported; 
%\item 40\% reduction in training data. does not scale up as more epochs. 
%\end{itemize}


% \xzlNote{Xu's version}
% AutoAssist \cite{zhang2019autoassist} proposes to train an assistant model to formulate informative data batches jointly with training the original (Boss) model. They have similar predictor design ideas with us, we both train a lightweight classier: logistic regression model and Naive Bayesian model. We also train it by target model's forward pass losses. 
% Other than that, we have different mechanism design. First, our simple model is trained by linguistic features extracted from current data batch instead themselves, so that our meta predictor is less likely to make the same mistakes as the big model. Second, even through their asynchronously training mechanism could improve utilization efficiency of hardware, the assistant and boss model in AutoAssist still depends on each other's results to prepare the training data by design. However, our three-stages training divides the meta predictor training and querying into two different stages, which eliminates the interdependence problem. Third, the loss threshold they use varies depending on the boss model status. This is a target-changing task for the assistant model, which actually hinders its performance. By contrast, in stage 1, the automatic loss threshold is fixed and the meta predictor is trained until fulfills our standard. Only meta predictor querying but no training in the last stage further improves the efficiency. In the end, our approach is focusing on finetuning instead of pretraining a large model, which is a more relevant problem to the NLP community.

% % \xzlNote{what is the similarity at a high level}
% However, it requires to do forward pass for each data instance while our Three-stage filtering is even able to further skip both forward and backward passes, which is crucial to further increase efficiency. 
% % \xzlNote{... which is crucial to efficiency}
% Moreover, training a Native Bayesian model is more efficient than training a linear SVM model as it has less parameters and only been updated in stage 2. \xzlNote{how important is this?}
% At a high-level, Assist model aims to prepare a core-set while we train the predictor play a role of filtering in an online-fashion. \xzlNote{can we say anything about the use case? efficiency?}
% As shown in Section \ref{sec:eval}, we focus on accuracy-efficiency trade-off and build a metric to represent it.


\iffalse
\note[YJ]{If we don't have enough space, we can move the following two paragraphs to the beginning of this section and briefly mention them as classical works on sample rewriting or selection, as these two methods are not mainly discussed in the context of deep learning.}


\paragraph{Aggressive-passive training (APT).} APT \cite{shalev2003online} targets online algorithms which receive data in a streaming fashion. It keeps the model's parameter unchanged when a new training example has a sufficiently low loss (being passive), otherwise updates the model (being aggressive). 
It shares our motivation -- training examples with low loss shall have a low impact on model parameters. Therefore, we only update the model with more important data. 
It, however, does not use this motivation to improve training efficiency by design. As it will calculate the loss for all the data. By contrast, our meta predictor could skip data instances without looking at their forward pass losses.
% \xzlNote{why? It skips model update if the loss is low}
% \textcolor{blue}{Error-driven learning \cite{OReillyMunakataFrankEtAl12} drives weights changes as a function of errors, which it directly tries to fix the problem.}

% \xzlNote{How is the below connected to ``data efficient'' training above?}



\paragraph{Perceptron}
% \note[YJ]{we can move the following discussion to the method section, as part of the connection with prior methods} 
Perceptron \cite{rosenblatt1958perceptron}, as an online algorithm, learns a binary classifier. It updates the model only on examples that it has misclassified. Our approach resonates with Perceptron, as we only update the target model on  data with high losses. Perceptron aims to get higher accuracy by making predictions on all examples. However, our approach aims to boost the accuracy-efficiency trade-off.
% \xzlNote{revise and move to S2}
\fi

\paragraph{Other training optimizations}
% \st{In terms of promoting the efficiency of finetuning, there are different methods have been proposed.}
include accelerating model convergence with the same amount of data, e.g. 
by varying the learning rate per weight \cite{jacobs1988increased,zeiler2012adadelta} or batch sizes \cite{smith2017don}.
% \xzlNote{how do the following works reduce training time?}
% \cite{jacobs1988increased, zeiler2012adadelta} suggests that every weight of a network should be given its own learning rate and these rates can vary over time. \cite{smith2017don} shows varying batch size can also achieve the same accuracy as tuning learning rate. 
% \paragraph{Model compression}
There also exist techniques for reducing training computation by reducing model parameters or finding a lightweight counterpart of a large model: 
pruning \cite{cui2019fine,mccarley2019structured,katharopoulos2018not},
% is simplifying a model by removing some components (channel, layer, and attention head, etc) in it. Integrating sparsity into self-attention \cite{cui2019fine}, applying structured pruning on BERT-based models \cite{mccarley2019structured} , and doing structured dropout during inference time.
% \xzlNote{citation missing? does that lead to model compression below?}
% \textbf{Distillation and Compact model}
knowledge distillation (KD) \cite{hinton2015distilling,sanh2019distilbert,jiao2019tinybert},
% is also a commonly used technique.
% that a compact model is trained under the guidance of a larger model. These models are also called student and teacher model respectively.
% DistillBERT \cite{sanh2019distilbert} pretrains a model from scratch solely through distillation. TinyBERT \cite{jiao2019tinybert} proposes a KD method specifically for Transformer-based models. By using KD, they are able to train a lightweight model achieving comparable accuracy.
quantization \cite{jacob2018quantization,micikevicius2017mixed},
% Training with fewer data precision is an another popular method that use less bits to save weights. Mixing full and half precision values \cite{micikevicius2017mixed} and quantizing model and input data to int8 \cite{jacob2018quantization} which save lots of training computation. 
low-rank approximation \cite{lan2019albert,ma2019tensorized}, and weights sharing \cite{dehghani2018universal,lan2019albert}. 
Our method is complementary to these optimizations and can be used in conjunction with them. % as we will show in \nameref{sec:eval}.
% \xzlNote{should say that we are complementary, e.g. we evaluate our method vs. layer freezing}

\iffalse
\paragraph{Active Learning} 
% \xzlNote{Xu should proof read this part}
Our goal is related to active learning but not the same: 
in an unsupervised setting, 
it down-selects unlabeled data for labeling and then training~\cite{settles2009active}. 
However, few active learning methods that employ a multistage process, 
which first trains a meta predictor in a \textit{supervised} fashion and then uses the predictor to filter data in an \textit{unsupervised} fashion. 
To this end, our idea can be extended to support active learning. 
\fi

%{\color{blue}Labeling a dataset is a time-consuming and expensive task. Active Learning \cite{settles2009active}’s goal is to filter data points to label such that the highest accuracy can be obtained given a fixed labeling budget. 
%
%Our approach has similarities to Active Learning in that both of them utilize the values of the loss function as the data valuation metric. Additionally, we also select the best data points during model training. Therefore, our method can also be used in AL when the oracle is replaced by our loss threshold and meta predictor. Ours is connected with AL.
%
%However, we have different goals with Active Learning. Our work belongs to supervised learning. We aim to filter the best subset of the whole labeled dataset to achieve comparable even better accuracy with training on the whole labeled dataset. Note that AL does not have the same goals and no prior AL work can achieve our goal.
%
%}



==> CamRd_IJCAI_efficient_NLP_Latex/summary.tex <==
\section{Conclusions}
\vspace{-1mm}
We present online data filtering, an efficient training mechanism for optimizing training data usage. We automatically maintain a loss threshold from model losses, then train and query a simple predictor to skip both forward and backward passes. So that unnecessary data instances will be filtered out and we achieve great accuracy-efficiency tradeoff. We formulate two algorithms under the Three-stage training method for three realistic and distinct NLP tasks, sentiment classification, QA/NLI, and paraphrase identification, which leads to consistent improvements over strong baselines.

==> CamRd_IJCAI_efficient_NLP_Latex/tab-baselines.tex <==
% !TeX root = main.tex

\begin{table}
\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/baselines.png}
%	\vspace{-2em}
%	\caption{Hyperparameters summary and their reasonable ranges}
	\caption{\color{blue}{Accuracy and training time of AutoAssist and Selection via Proxy. Training time normalized to TrainAll of the same benchmark. Only the AGOT-optimal results are shown. (This table can be merged with the following benchmarks table.)}}
	\label{tab:baselines}
\end{table}

==> CamRd_IJCAI_efficient_NLP_Latex/tab-complexity.tex <==
% !TeX root = main.tex

\begin{table}
\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/complexity.png}
%	\vspace{-2em}
%	\caption{Hyperparameters summary and their reasonable ranges}
	\caption{\color{blue}{Fractions of skipped training computation of our method. (This table can be merged with Table \ref{tab:skipratio}).)}}
	\label{tab:complexity}
\end{table}

==> CamRd_IJCAI_efficient_NLP_Latex/tab-e2e-combined.tex <==
% !TEX root = main.tex
\begin{table*}[t]
	\centering
	\includegraphics[width=0.95\textwidth{}]{./figs/e2e-combined-xu.pdf}
	\vspace{-2mm}
	\caption{Our method as compared to the baselines. For our method, only the AGOT-optimal results are shown.}
	\label{tab:e2e-combined}
	\vspace{-3mm}
\end{table*}
	

==> CamRd_IJCAI_efficient_NLP_Latex/tab-e2e.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/e2e}
%	\vspace{-2em}
	\caption{Accuracy and training time of our method and the baselines. 
	Training time normalized to \textit{TrainAll} of the same benchmark. 
	For our methods, only the AGOT-optimal results are shown.}
	\label{tab:comparisons}
%	\vspace{-2em}
\end{table}
	

==> CamRd_IJCAI_efficient_NLP_Latex/tab-epochs.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/epochs.pdf}
	\vspace{-2mm}
	\caption{
	Accuracy and training time ($T_{norm}$) as the epoch count ($N_{epochs}$) grows, showing that our method yields increasingly higher efficiency in additional epochs. 
	$T_{norm}$ is normalized to the time of \textit{TrainAll} of the same $N_{epochs}$. 
% 	The results show that our method yields increasingly higher efficiency as the model is trained for additional epochs. 
%	For our methods, only the AGOT optimal results are shown.
	}
	\label{tab:epochs}
	% \vspace{-2em}
\vspace{-3mm}
\end{table}


==> CamRd_IJCAI_efficient_NLP_Latex/tab-freeze.tex <==
% !TeX root = main.tex

\begin{table}[t]
\scalebox{0.8}{
\centering
\begin{tabular}{lllll}
\hline
\textbf{Benchmarks}& \textbf{SST2} & \textbf{QNLI} & \textbf{QQP} & \textbf{AMZ} \\
\hline
\textit{TrainAll}+LF &88.99/1.00 &82.17/1.00  &86.64/1.00 &94.29/1.00 \\
Ours+LF &88.53/0.21 &81.15/0.57 &85.03/0.52 &92.79/0.14 \\
\hline
\end{tabular}
}
\vspace{-2mm}
\caption{Accuracy and training time of our method and
\textit{TrainAll} with layer freezing. Training time normalized to \textit{TrainAll}+LF of the same benchmark}
\label{tab:freeze}
\vspace{-5mm}
\end{table}


==> CamRd_IJCAI_efficient_NLP_Latex/tab-hyperparam.tex <==
% !TeX root = main.tex

\begin{table}
\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/hyperparameters.pdf}
	\vspace{-1em}
%	\caption{Hyperparameters summary and their reasonable ranges}
	\caption{A summary of hyperparameters. 
	The value range column shows concrete values used in evaluation.}
	\label{tab:hyperparam}
 \vspace{-3mm}
\end{table}

==> CamRd_IJCAI_efficient_NLP_Latex/tab-overview.tex <==
% !TeX root = main.tex
\begin{table}[t]
		\centering
	\includegraphics[width=0.48\textwidth]{figs/highlight-res-docx}
		\vspace{-6mm}
	\caption{Our method significantly reduces training time (in hours) while achieving accuracies comparable to training with all the data (\textit{TrainAll}). Details in \S\ref{sec:eval}.
	GPU: Nvidia RTX 2080Ti.}
	\label{tab:highlight-res}
		\vspace{-4mm}
\end{table}



==> CamRd_IJCAI_efficient_NLP_Latex/tab-passcost.tex <==
\begin{table}
\centering
\begin{tabular}{llllll}
\hline
\textbf{Datasets} & \textbf{Backward/Forward pass cost}\\
\hline
SST2 & 2.28 \\
QNLI & 2.07 \\
QQP & 2.25 \\
Amazon Polarity & 2.19 \\
\hline
\label{tab:pass-cost}
\end{tabular}
\caption{
The runtime ratio of backward pass cost over forward pass cost. The backward passes of all four datasets run more than 2 times slower than forward passes.
}
\end{table}

==> CamRd_IJCAI_efficient_NLP_Latex/tab-random.tex <==
% !TeX root = main.tex

\begin{table}[t]
	\centering
	\includegraphics[width=0.3\textwidth]{./figs/random.pdf}
		\vspace*{-1mm}
%	\caption{Filtering training data via loss threshold is Random vs Fix threshold}
	\caption{Using loss thresholds for skipping data is superior to skipping  the same amount of data but is randomly picked. FT means using a fixed threshold; Three-stage uses an automatic threshold. Numbers are accuracy.}
	\label{tab:cmp-random}
		\vspace{-5mm}
\end{table}

==> CamRd_IJCAI_efficient_NLP_Latex/tab-skipratio.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/skipratio3.pdf}
%	\vspace{-2em}
	\caption{Fractions of skipped training computation of our method and the baselines. For our methods, only the AGOT-optimal results are shown.}
	\label{tab:skipratio}
%	\vspace{-2em}
\end{table}

% \begin{table}
% \centering
% \scalebox{0.7}{
% \begin{tabular}{lllllll}
% \hline
% \textbf{C} & & \textbf{SST2} & \textbf{QNLI} & \textbf{QQP} & \textbf{AMZ} \\
% \hline
% Fixed & 0.1 & 90.9 & 88.9 & 88.7 & 95.2 \\
% Threshold & 0.3 & 90.9 & 88.9 & 88.7 & 95.2 \\
% & 0.5 & 90.9 & 88.9 & 88.7 & 95.2 \\
% & 0.7 & 90.9 & 88.9 & 88.7 & 95.2 \\
% \hline
% Ours & Auto threshold & 90.48 & 84.24 & 86.94 & 93.67\\
% \hline
%  & Three stages & 91.17 & 87.72 & 88.05 & 94.99 \\
% \hline
% \label{tab:skipratio}
% \end{tabular}
% }
% \caption{
% Fractions of skipped training computation of our method and the baselines. For our methods, only the results with highest AGOT are shown
% }
% \end{table}

==> CamRd_IJCAI_efficient_NLP_Latex/terms.tex <==
% !TeX root = main.tex

% -------------------TERMS -------------------

\newcommand{\secenv}{secure environment}
\newcommand{\unsecenv}{normal environment}

\newcommand{\se}{secure world}
\newcommand{\te}{secure world}
\newcommand{\Te}{Secure world}
\newcommand{\Se}{Secure world}
\newcommand{\nw}{normal world}
\newcommand{\sw}{secure world}

\newcommand{\mobile}{mobile SoC}
\newcommand{\Mobile}{Mobile SoC}
\newcommand{\bL}{big.LITTLE}


%\newcommand{\sys}{TZGPU}
%\newcommand{\sys}{TinyStack}
\newcommand{\sys}{STI}
%\newcommand{\sys}{\textbf{\textit{STI}}}
\newcommand{\psb}{\textbf{power sandbox}}
\newcommand{\dbt}{\textbf{transkernel}}
\newcommand{\enigma}{\textbf{enigma}}
\newcommand{\drv}{\textbf{driverlet}}

%\newcommand{\teedriver}{Drvlet}
\newcommand{\teedriver}{driverlet}
\newcommand{\Teedriver}{Driverlet}
\newcommand{\teedrivers}{driverlets}


%\newcommand{\systz}{TinyStack-TZ}
\newcommand{\mm}{memory manager}

%\newcommand{template}{trace template}
%\newcommand{Template}{Trace template}
\newcommand{\template}{interaction template}
\newcommand{\Template}{Interaction template}


\newcommand{\ioctl}{\texttt{ioctl}}
\newcommand{\register}{\texttt{reg}}
\newcommand{\dwait}{D$_{wait}$}
\newcommand{\irqwait}{\texttt{irq\_wait}}
\newcommand{\val}{\texttt{val}}

\newcommand{\armtz}{arm trustzone}
\newcommand{\tz}{trustzone}
\newcommand{\TZ}{TrustZone}
\newcommand{\ARMTZ}{ARM TrustZone}
%\newcommand{\tee}{TEE}
\newcommand{\tfm}{transformer}
\newcommand{\Tfm}{Transformer}

\newcommand{\tee}{trusted execution environment}

%% ----------------------------------------------

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

PROJECT = main

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
CC = pdflatex # xelatex ## pdflatex 
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	$(CC) $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	$(CC) $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	$(CC) $(PDFLATEX_FLAGS) $(PROJECT)
	grep --color auto -e "Warning" obj/$(PROJECT).log


==> fig-overview.tex <==
% !TeX root = main.tex
\begin{figure}[t]
	%	\centering
	\includegraphics[width=0.48\textwidth]{./figs/highlight-res1}
	%	\vspace*{-2em}
	\caption{Our method significantly reduces training time (columns, right y-axis) while achieving accuracies (lines, left y-axis) comparable to training with all the data. Benchmark details in \nameref{sec:eval}.
	GPU: Nvidia RTX 2080Ti.}
	\label{fig:highlight-res}
	%	\vspace{-5mm}
\end{figure}



==> recycle/recycle-eval.tex <==
\autoref{tab:pass-cost} shows the ratios of backward pass cost over forward pass cost. By these ratios, we can calculate the total amount of run time and our equations can be easily applied to a different machine once its cost ratio is also known.

Intuitively, our compute saving grows with higher skip ratio (both forward and backward passes) and the shorter stage 1 and 2. To quantify the total amount of run time, we have following assumptions:\\
1. Assume on $p\%$ of data we skip backward passes only
and on $q\%$ of data we skip both forward and backward passes.\\
2. Assume a forward pass takes GFLOPs = $X$ and a backward pass has GFLOPs = $Y$. \\
3. Automatic threshold's total computation is $S_{auto}$ and three-stage's total computation is $S_{3-stage}$.
\begin{equation}
\begin{split}
&S_{auto} = p*X+(1-p)(X+Y)\\
&S_{3-stage} = p*X+(1-p-q)(X+Y)
\end{split}
\end{equation}
Because we will use the normalized run time, which within $[0, 1]$, we take $X$ = 1 and different $Y$ for different datasets. For specific numbers, see Table 6.
In \autoref{tab:platform} and \autoref{tab:epochs}, the listed run time is normalized by $S' / S_{vanilla}$, where $S'$ is the total computation of Fixed threshold, Automatic and Three-stage training.

% The comparison with these two baseline methods mainly focuses on prediction performance as no explicit or very preliminary methods are applied to improve efficiency.
% \note[YJ]{I am not sure how to merge the following items}
% \begin{itemize}
% \item Vanilla (train with all data)
% \item Hand-picked thresholds (sweep, \st{optimal}). 
% \item \textcolor{blue}{I think 2-stage should goes to the ablation study} Stage 1 and 2 (automatic threshold; no predictor) 
% \end{itemize}
% \textcolor{blue}{I think LF should be our contribution, instead of as a baseline} Further: +LF. baselines enhanced with layerwise freezing, a common optimization for LM finetuning.

% \paragraph{Evaluation metrics}
% \note[YJ]{We should summarize the evaluation metrics, including the ones for prediction performance and the ones for training efficiency. As we have comparable prediction performance, it should not be our major focus when we present the results in section 4.2}



We take accuracy and forward/backward skip ratio together as metrics to measure how good an result is. We further calculate run time based on skip ratios and take it as the metric of efficiency. For comprehensive comparisons, high accuracy with long run time is not good and vice versa.

reports the accuracy (y-axis) and running time (x-axis) with the hyperparameter settings that achieve the highest accuracy on four datasets. 
To make the x-axis more readable, we normalize the running times by the elapsed real time of training with all examples. 


==> recycle/recycle-intro-xu.tex <==
% !TeX root = main.tex

\section{Introduction}
% Starting Point
%% Deep learning hot in NLP
Deep learning has shown remarkable success in many natural language processing tasks, but the current paradigm requires further efficiency boost. Large models, such as BERT, RoBERTa and GPT3, have become the \textit{de facto} models used in many NLP tasks. However, the prohibitively pretraining expense limits the model pretraining to only a few industry labs. There have been many research focus on pretraining  a large language model with much less resources and budget. \\
%% Finetuning in NLP takes time and resources
However, the finetuning which is usually considered much cheaper than the pretraining lacks enough attention to boost its efficiency. In this paper, we focus on the problem of increasing the finetuning efficiency in NLP tasks.
%% Highlight of the paper: 1 epoch; A large number of training data
We show that just 1 epoch of finetuning could achieve comparable accuracy with only about 40\% - 50\% training data, which could save a significant amount of training time and resources.\\
% Why care about efficiency
The reason why we care about the efficiency of finetuning lies in it has at least 4 advantages: 1. Efficient finetuning could save a large amount of training budget. 2. Finetuning could happen in many tasks 3. Efficient finetuning promotes green NLP. 4. Finetuning is data even user specific. it saves time and efforts. \textcolor{blue}{// Notes: should elaborate one more sentence in each point, but it's easily looks redundant and unprofessional.}\\
% Different methods proposed
In terms of promoting the efficiency of finetuning, there are different methods have been proposed. First, some papers propose the efficient training algorithms to reduce training cost. Second, some papers focus on reducing model parameters or finding a lightweight counterpart of a large model, However, not many papers care about reducing training cost by reducing the training data, where large research chances are ignored. Third, some papers propose methods that weight different data differently. But these methods have lots of computing overhead that consumes more time to train the classifier.\\
% Our research question
Many previous works have shown that not all the data points are equally important, so we take the losses of forward propagation as a standard to weight the current training data. Unlike the previous papers, we apply a very lightweight Native Bayesian classifier to classify whether the current data point should be skipped and we also propose a 3-stage training recipe that gradually train the NLP model along with the classifier. In terms of training data that makes an impact, our approach has similarities with the Perceptron algorithm, which only updates the model based on the data that it makes mistakes and puts the correctly classified data aside. \\
% Contributions
The contribution of this work is four-fold:(1) we propose the 3-stage training recipe to train the NLP model and a Naive Bayesian classifier that can achieve comparable model accuracy with significantly less training data (2) different from the expensive data weighting methods proposed in other papers, we adopt lightweight Native Bayesian classifier to decide the data skipping. Its efficiency has been proofed by the experiments and explanations in the following section (3) we propose adaptive loss threshold method to train the Naive Bayesian classifier in stage 1, which helps the classifier does online learning along with the NLP model training. (4) we evaluated the proposed method with XX models: ...., on XX datasets via both quantitative and qualitative evaluations.\\


==> recycle/recycle-related.tex <==
% !TeX root = main.tex

\section{Related work}
\paragraph{Efficient training techniques}\\
In terms of promoting the efficiency of finetuning, there are different methods have been proposed. First, some papers propose training tricks to reduce training time. \cite{jacobs1988increased, zeiler2012adadelta} suggests that every weight of a network should be given its own learning rate and these rates can vary over time. \cite{smith2017don} shows varying batch size can also achieve the same accuracy as tuning learning rate. 
Second, some papers focus on reducing model parameters or finding a lightweight counterpart of a large model.
\paragraph{Model compression}\\
\textbf{Pruning} Pruning is simplifying a model by remove some components (channel, layer, and attention head, etc) in it.  \cite{cui2019fine} integrates sparsity into self-attention to enhance the fine-tuning performance of BERT. \cite{mccarley2019structured} apply structured pruning and distillation on BERT-based model. \cite{fan2019reducing} proposes structured dropout method: LayerDrop pruning during inference time.
\textbf{Distillation and Compact model}
Knowledge Distillation \cite{hinton2015distilling} is a technique that a compact model is trained under the guidance of a larger model. These models are also called student and teacher model respectively. DistillBERT\cite{sanh2019distilbert} pretrains a model from scratch solely through distillation. TinyBERT\cite{jiao2019tinybert} proposes a knowledge distillation method specifically for Transformer-based models. They also aim to train a smaller model having less computation cost. DistillBERT model has six layer and TinyBERT has four layers.
\textbf{Quantization} Training with fewer data precision is an another popular method, \cite{micikevicius2017mixed} proposes mixing full and half precision values and \cite{jacob2018quantization} quantizes model and input data to int8 which save lots of training computation. 
\textbf{Low-rank approximation} \cite{lan2019albert, ma2019tensorized} and \textbf{Weights sharing} \cite{dehghani2018universal, lan2019albert} are also important techniques.
However, not many papers care about reducing training cost by reducing the training data, where large research chances are ignored. 
% Our research question
\paragraph{Redundancy in training sets}\\
Previous paper \cite{katharopoulos2018not} shows that there are much redundancy in data instances and model components. Not each of them is equally important. Some data and model components can be removed without hurting or even improving the performance due to the increased model flexibility. \cite{birodkar2019semantic} shows there are at least 10\% redundant data in object recognition benchmarks. The existing redundancy in training sets motivates us to propose a training mechanism more data-efficient.
\paragraph{Data-efficient training}\\
Prior work on data selection like \cite{wang2020optimizing} proposes using reinforcement learning to train a scorer that weights data to maximally benefit learning. But it has lots of computing overhead and they care about finding how much attention the model should pay to different data. \cite{xia2021sample} adopts interval estimation of losses to find the correct labels to improve learning on noisy labels. But we are working on tasks that have clear labels instead of updating the model with labels more likely to be correct. Other data-selection training methods share similar goal with us: CRAIG \cite{mirzasoleiman2020coresets} can find a small subset such that the weighted sum of the gradients of its elements closely approximates the full gradient over the full training set. \cite{zhang2019autoassist} proposes to train an Assistant model, a linear model to filter out less informative instances, jointly the original (Boss) model. \cite{coleman2019selection} proposes to simplify the big target model to a small proxy model then use it to select core-set which is used to train the target model. 
Essentially, above papers' goals and approaches are not same as ours.
CRAIG \cite{mirzasoleiman2020coresets} and model proxy \cite{coleman2019selection} are data-prepossessing methods before the large model starts training. But in our method, both Automatic filtering and Three-stage filtering are training along with the target model. \cite{zhang2019autoassist} also train a linear SVM model during Boss model training, However, it requires to do forward pass for each data instance while our Three-stage filtering is even able to further skip both forward and backward passes. Moreover, training a Native Bayesian model is more efficient than training a linear SVM model as it has less parameters and only been updated in stage 2. In high-level, Assist model aims to prepare a core-set while we train the predictor play a role of filtering in an online-fashion. As shown in Section 4, we focus on accuracy-efficiency trade-off and build a metric to represent it. 
\paragraph{Aggressive-passive training.}(APT) \cite{shalev2003online} targets online algorithms which receive data in a streaming fashion. It keeps the model's parameter unchanged when a new training example has a sufficiently low loss (being passive), otherwise updates the model (being aggressive). 
It shares our motivation -- training examples with low loss shall have low impact on model parameters. Therefore, we only update the model with more important data. 
It, however, does not use this motivation to improve training efficiency as it will not skip training data.
\textcolor{blue}{Error-driven learning \cite{OReillyMunakataFrankEtAl12} drives weights changes as a function of errors, which it directly tries to fix the problem.}

==> tab-baselines.tex <==
% !TeX root = main.tex

\begin{table}
\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/baselines.png}
%	\vspace{-2em}
%	\caption{Hyperparameters summary and their reasonable ranges}
	\caption{\color{blue}{Accuracy and training time of AutoAssist and Selection via Proxy. Training time normalized to TrainAll of the same benchmark. Only the AGOT-optimal results are shown. (This table can be merged with the following benchmarks table.)}}
	\label{tab:baselines}
\end{table}

==> tab-complexity.tex <==
% !TeX root = main.tex

\begin{table}
\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/complexity.png}
%	\vspace{-2em}
%	\caption{Hyperparameters summary and their reasonable ranges}
	\caption{\color{blue}{Fractions of skipped training computation of our method. (This table can be merged with Table \ref{tab:skipratio}).)}}
	\label{tab:complexity}
\end{table}

==> tab-e2e.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/e2e}
%	\vspace{-2em}
	\caption{Accuracy and training time of our method and the baselines. 
	Training time normalized to \textit{TrainAll} of the same benchmark. 
	For our methods, only the AGOT-optimal results are shown.}
	\label{tab:comparisons}
%	\vspace{-2em}
\end{table}
	

==> tab-passcost.tex <==
\begin{table}
\centering
\begin{tabular}{llllll}
\hline
\textbf{Datasets} & \textbf{Backward/Forward pass cost}\\
\hline
SST2 & 2.28 \\
QNLI & 2.07 \\
QQP & 2.25 \\
Amazon Polarity & 2.19 \\
\hline
\label{tab:pass-cost}
\end{tabular}
\caption{
The runtime ratio of backward pass cost over forward pass cost. The backward passes of all four datasets run more than 2 times slower than forward passes.
}
\end{table}

==> tab-skipratio.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/skipratio3.pdf}
%	\vspace{-2em}
	\caption{Fractions of skipped training computation of our method and the baselines. For our methods, only the AGOT-optimal results are shown.}
	\label{tab:skipratio}
%	\vspace{-2em}
\end{table}

% \begin{table}
% \centering
% \scalebox{0.7}{
% \begin{tabular}{lllllll}
% \hline
% \textbf{C} & & \textbf{SST2} & \textbf{QNLI} & \textbf{QQP} & \textbf{AMZ} \\
% \hline
% Fixed & 0.1 & 90.9 & 88.9 & 88.7 & 95.2 \\
% Threshold & 0.3 & 90.9 & 88.9 & 88.7 & 95.2 \\
% & 0.5 & 90.9 & 88.9 & 88.7 & 95.2 \\
% & 0.7 & 90.9 & 88.9 & 88.7 & 95.2 \\
% \hline
% Ours & Auto threshold & 90.48 & 84.24 & 86.94 & 93.67\\
% \hline
%  & Three stages & 91.17 & 87.72 & 88.05 & 94.99 \\
% \hline
% \label{tab:skipratio}
% \end{tabular}
% }
% \caption{
% Fractions of skipped training computation of our method and the baselines. For our methods, only the results with highest AGOT are shown
% }
% \end{table}
